Improving Zero-shot Generalization and Robustness of Multi-modal Models

Multi-modal image-text models such as CLIP and LiT have demonstrated impressive performance on image classification benchmarks and their zero-shot generalization ability is particularly exciting. While the top-5 zero-shot accuracies of these models are very high, the top-1 accuracies are much lower (over 25% gap in some cases). We investigate the reasons for this performance gap and find that many of the failure cases are caused by ambiguity in the text prompts. First, we develop a simple and efficient zero-shot post-hoc method to identify images whose top-1 prediction is likely to be incorrect, by measuring consistency of the predictions w.r.t. multiple prompts and image transformations. We show that our procedure better predicts mistakes, outperforming the popular max logit baseline on selective prediction tasks. Next, we propose a simple and efficient way to improve accuracy on such uncertain images by making use of the WordNet hierarchy; specifically we augment the original class by incorporating its parent and children from the semantic label hierarchy, and plug the augmentation into text prompts. We conduct experiments on both CLIP and LiT models with five different ImageNet-based datasets. For CLIP, our method improves the top-1 accuracy by 17.13% on the uncertain subset and 3.6% on the entire ImageNet validation set. We also show that our method improves across ImageNet shifted datasets, four other datasets, and other model architectures such as LiT. The proposed method is hyperparameter-free, requires no additional model training and can be easily scaled to other large multi-modal architectures. Code is available at https://github.com/gyhandy/Hierarchy-CLIP.

==> content.tex <==
% \usepackage{breqn}
% \usepackage{amsmath}

\begin{abstract}
Multi-modal image-text models such as CLIP and LiT have demonstrated impressive performance on image classification benchmarks %achieved tremendous success in various domains
and their zero-shot generalization ability is particularly exciting. %as it allows models to be quickly deployed to new domains without any additional training. 
While the top-5 zero-shot accuracies of these models are very high, the top-1 accuracies are much lower (over 25\% gap in some cases). We investigate the reasons for this performance gap and %propose a simple method to improve zero-shot generalization and robustness. 
find that many of the failure cases are caused by ambiguity in the text prompts. %embedding.  
First, we develop a simple and efficient zero-shot post-hoc  method to identify images whose top-1 prediction is likely to be incorrect, by measuring consistency of the predictions w.r.t. multiple prompts and image transformations. 
We show that our procedure better predicts mistakes, outperforming the popular max logit baseline on selective prediction tasks. 
Next, we propose a simple and efficient way to improve accuracy on such uncertain images by making use of the WordNet hierarchy; specifically we augment the original class by incorporating its parent and children from the semantic label hierarchy, and plug the augmentation into text promts.  %and  to enhance the robustness, and that leads to up to 17.13\% improvement on accuracy.  
 We conduct experiments on both CLIP and LiT models with five different ImageNet-based datasets. For CLIP, our method \textbf{improves the top-1 accuracy by 17.13\% on the uncertain subset and  3.6\% on the entire ImageNet validation set.} We also show that our method improves across ImageNet shifted datasets and other model architectures such as LiT.
% but may also their robustness, generalization, and calibration, which can lead to more reliable and trustworthy decisions. 
%Overall, our proposed method shows significant improvement on accuracy and generalization for zero-shot inference. 
\textbf{Our proposed method is hyperparameter-free, requires no additional model training and can be easily scaled to other large multi-modal architectures.}
% Code for our experiments is opensourced at \emph{link hidden for anonymity.}
%In the zero-shot setting, top-1 zero-shot inference accuracy is much lower than top-5 (over 25\% gap), which shows the instability of the decision. We first analyzed and summarized that most failure cases are caused by noise and ambiguity in text prompt embedding. Then we propose 1) a zero-shot confidence estimation via self-consistency to provide the model an "additional choice": "not sure" during decision and improves the selective prediction performance by over 7\% than baseline methods. 2) a top-down and bottom-up prompt augmentation using WordNet hierarchy to improve the performance on the selected un-confident samples. We conduct experiments on both CLIP and LiT models with five different ImageNet-based datasets, and our method achieves at most +17.13\% and +3.6\% improvement on unstable subset and whole ImageNet, respectively, verifying the effectiveness of our method.  

%Multi-modal’s generalization and robustness is critical for deployment of the model to products. %Currently the multi-modal’s zero-shot accuracy is still much lower than the production standard. 
% Motivated by the big gap between top-1 accuracy and top-5 accuracy in zero-shot ImageNet inference, we investigated the failure modes and found that the model's prediction is very sensitive to text prompts. 
% Thus we develop a simple but efficient zero-shot post-hoc method to identify images where top prediction is unstable w.r.t. prompts. 
% For those unstable predictions, we make use of WordNet hierarchy to augment class labels to enhance the robustness, and that leads to up to 17.13\% improvement on accuracy.  
% We show our method make consistent improvement on other ImageNet shifted datasets and other model architectures.
% % but may also their robustness, generalization, and calibration, which can lead to more reliable and trustworthy decisions. 
% Overall, our proposed method shows significant improvement on accuracy and generalization for zero-shot inference. 
% Our framework is hyperparameter-free, training-free, post-processing method that can be easily extended to other multi-modal architectures. 

\end{abstract}
% \begin{abstract}
% Vision-language models encode \{image, text\} pairs in a common embedding space, which allows zero-shot generalization to downstream tasks like image classification via text prompting. 
% One of the major blockers to deploying zero-shot inference with pretrained vision-language multi-modal, e.g.,  CLIP, LiT, is that their top-1 accuracy is significantly lower than top-5, which shows the instability of model performance. 
% For instance, CLIP reaches 89.4\% top-5 accuracy, while its top-1 accuracy is only 64.2\% in ImageNet classification. 
% In this paper, we propose to re-rank the initial top-5 labels list, with the expectation that the ground-truth labels receive high ranks, thereby boosting the top-1 accuracy. 
% Specifically, we first identify the potential uncertain predictions, and then craft a simple yet effective prompt to re-rank their initial top-5 label lists. 
% Different from existing prompt engineering and learning, which try to adapt context words or learn context embedding vectors, we fix the context words in our prompts, and only change the ``\{class\}'' in the prompt template ``\texttt{a photo of \{class\}}''. 
% More concretely, we directly replace ``\texttt{class}'' in the prompt template by the concatenation of ``\texttt{\{parent, class, children\}}'' from the WordNet hierarchy, this simple modification makes label semantics transfer among parent-child in the hierarchy and enhances correct predictions while suppressing wrong predictions.
% The proposed re-ranking method is a post-processing step, which is independent of the upstream models and requires no training data, and consistently improves the top-1 accuracy over all test sets.
% \end{abstract}


% \vspace{-15pt}
% \vspace{-2em}
\section{Introduction}
% \vspace{-1em}
Vision-language multi-modal models trained on large-scale data have achieved significant success in numerous domains and have demonstrated excellent zero-shot generalization ability \citep{radford2021learning,zhai2022lit,pham2021combined,jia2021scaling,ramesh2021zero,ge2022dall}.
% CLIP \citep{radford2021learning}, LiT \citep{zhai2022lit}, BASIC \citep{pham2021combined}, ALIGN \citep{jia2021scaling}. 
%
Given a test image and a set of candidate class labels, one can compute the similarity between the embedding of the image and the embedding of each of the candidate class labels, and predict the class as the one with the highest similarity. 
The zero-shot top-$1$ accuracy for ImageNet using CLIP variants (CLIP ViT-L) matches the performance of the original ResNet model trained from scratch. 
%
Recently, CLIP has been found to be more robust to distribution shift than ResNet, achieving good performance on ImageNet-V2 \citep{recht2019imagenet}, ImageNet-R \citep{hendrycks2021many}, ImageNet-A \citep{hendrycks2021natural}, and ImageNet-Sketch \citep{wang2019learning}.

We noticed a large gap between the top-$1$ accuracy and top-$5$ accuracy, 64.2\% vs. 89.4\% respectively, revealing potential headroom for improvement. 
We investigated the cases where the top-$1$ prediction was incorrect but the top-$5$ prediction was correct, and identified several typical failure modes. 
Despite the well-known multi-label issues in ImageNet \cite{beyer2020we}, we found many of the remaining failure cases are caused by noise and ambiguous text prompts related to the WordNet hierarchical structure of ImageNet.
Some class names are quite general so that the model cannot correctly match images from their specific subclasses. For example, the hot-air balloon images belonging to the ``balloon'' class were misclassified as ``airship'', see Figure \ref{fig:failure-mode} middle.
On the other hand, some class names are too specific such that the model fails to correlate them with their more generic super-classes. For example, 96\% of images with ground truth label ``tusker'' are wrongly classified as other elephant classes such as ``Asian elephant'', see Figure \ref{fig:failure-mode} left. 
The failure modes analysis suggests that the text encoder is very sensitive to inputs and as a result, the overall classification lacks robustness. %, 

Inspired by these observations, we propose to first identify the subset of images whose top-1 prediction is likely to be incorrect, and then improve the accuracy for those images by a principled framework to augment their class labels by WordNet hierarchy.
To estimate whether an image has an incorrect prediction, i.e., to estimate the prediction confidence, we use the consistency of predictions under different text prompt templates and image augmentations as a signal for prediction confidence estimation.
%the low confidence subset of predictions that suffer from the instability issue.
% For the images in the identified low confidence subset, we propose a principled framework to increase the prediction accuracy by improving the text prompts using the WordNet hierarchy.
% modify their prompts to improve the accuracy  and consequently the robustness.  
Although prediction confidence estimation has been well studied in single-modal classification models, we found those commonly used confidence scores, maximum softmax probability \citep{hendrycks2016baseline} and maximum logit score \citep{hendrycks2019scaling}, are not always reliable for the multi-modal CLIP and LiT models due to the poor calibration of the logits scores. 
For example, among the 1K classes in ImageNet, the class with the greatest mean logit value (computed as the cosine similarity between image and text embeddings) is ``fig'' (the fruit).
%, and the one with the lowest mean logit value is ``desert grassland whiptail lizard''. 
Though we don't have access to CLIP private training data, 
we hypothesize that this might be due to ``fig'' being a common abbreviation for ``figure'', which frequently occurs in the training data and thus includes many non-fruit illustrations.  


%%%%%
%%%%% Fig.1
%%%%%
\begin{figure*}[ht]
% \vspace{-30pt}
\centering
\includegraphics[width=0.95\textwidth]{figure_failure_modes_update.pdf}
% \vspace{-1em}
\caption{Typical failure modes in the cases where top-5 prediction was correct but top-1 was wrong. %\todo{check copyright}
% : 1) class name does not explicitly specifies the super-class name; 2) class names are ambiguous; 3) class names are confounded by an adjective, ignoring the noun.
}
\label{fig:failure-mode}
% \vspace{-1.5em}
\end{figure*}


In this work, we first propose a simple yet efficient zero-shot confidence estimation method better suited for CLIP, based on predictions' self-consistency over different text prompts and image perturbations. %\textit{Self-consistency} was previously used for improving the reasoning accuracy of large language models \citep{wang2022self}. 
\citep{wang2022self} proposed using self-consistency among multiple model outputs to improve the reasoning accuracy of large language models. 
Here we extend the idea for confidence estimation in multi-modal models by measuring \emph{consistency of predictions under multiple input text prompts and image transformations}. Our method is effective at predicting mistakes;  
the identified low confidence subset has significantly lower top-1 accuracy (21.58\%) than the average accuracy (64.18\%). 
Next, to improve the accuracy for the low confidence subset, we develop a %top-down and bottom-up 
label augmentation technique using WordNet label hierarchy. Our method leverages semantic information from ancestors (top-down) as well as children (bottom-up) and improves the top-1 accuracy of the subset to 38.71\% (17.13\% improvement).
Our method not only improves model accuracy, but also model robustness, improving on ImageNet variants with distribution shift such as ImageNet-v2, ImageNet-R, ImageNet-Adversarial and Imagenet-Sketch. %other natural distributional shift datasets.
%Our framework is a hyperparameter-free, training-free, post-processing method that can be easily extended to other multi-modal models.

The main contributions of this work are:
\begin{compactitem}
    \item We identified several failure modes for zero-shot ImageNet classification using multi-modal models, and our findings suggest that the text encoder is very sensitive to prompts. To improve the prediction accuracy, prompts need to be better designed. 
    \item We propose a simple yet efficient zero-shot confidence score that is better suited for multi-modal models, based on predictions' self-consistency under different text prompts and image perturbations. 
    \item We develop a label augmentation technique that uses both ancestor and children labels from WordNet. By applying the label augmentation to the previously identified low confidence subset of images, we significantly improve their prediction accuracy. 
\end{compactitem}



% One of the major blockers to deploying zero-shot inference with pretrained vision-language multi-modal, e.g., , is that their top-1 accuracy is much lower than top-5, which shows the instability of model performance. 
% %
% For instance, CLIP reaches 89.4\% top-5 accuracy, while its top-1 accuracy is only 64.2\% in zero-shot setting. 
% %
% The large gap between top-5 and top-1 accuracy motivates us the natural questions: (1) How can we identify those incorrect top-1 predicted examples. (2) Given that the correct label is already within the top-5 matches in most cases, can we design a method to re-rank the top-5 label list, such that the groundtruth label floats up therefore reaching improved top-1 accuracy? 
% %
% In this paper, we focus on the re-ranking problem. 

% Re-ranking is widely studied in numerous areas including instance retrieval, multimedia, recommendation systems, NLP, computer vision and machine learning, to name a few \cite{collins2005discriminative,mei2014multimedia,shen2012object,zhong2017re}. 
% %
% Given an initial ranking list of retrieved instances, it aims to re-rank and increase the ranks of relevant  instances higher while pushing the ranks of less relevant ones lower. 
% %
% The main advantage of re-ranking is that it is independent of the upstream ranking methods, and can be implemented as a post-processing step of any initial ranking results. 


% Recent pre-trained image-text models have demonstrated zero-shot transfer learning capability in numerous vision tasks such as image classification: by comparing text embedding ``\texttt{a photo of \{class\}}'' with the image embedding, the ``\texttt{class}'' with the largest similarity is the predicted category of the image.
% %
% However, it is shown in [???, coop, prompt engineering] that the downstream object recognition performance relies largely on the input prompt.
% %
% In other words, a slightly change of the input wording affects the recognition accuracy of these models significantly.
% %
% AS such, numerous approaches have been developed to manually craft prompts or automatically learn prompts to adapt pre-trained image-text models for the downstream object recognition task. 
% %
% While existing work on contextual word engineering [???], sentence structure crafting [???] or contextual token learning [???] makes significant improvement on classification accuracy, they all fix the object label space, and only adapt the contextual surrounding words in the prompts.
% %
% In this paper, we do the opposite: fix the context, but adjust the labels. 

% %HERE
% In this work, we study how to perform zero-shot classification of pre-trained text-image models by exploiting the hierarchical structure of real world labels. 
% %
% Superficially, we replace ``\texttt{class}'' in the prompt template by the concatenation of ``\texttt{\{parent, class, children\}}'' from the WordNet hierarchical tree, and show this simple prompt modification leards consistent improvements over all our test datasets. 
% %
% Our motivation comes from the empirical observations.
% %
% During the training process of an image-text model, the same object are labeled at different granularities: e.g., some doberman are labeled as the specific category ``doberman'', while others are simply labeled as the more generic ``dog''. 
% %
% The rich label hierarchy is implicitly encoded in the pre-trained models. 
% %
% In the inference stage, by utilizing the label hierarchy, label semantics among children-parent have the potential to be transferred, therefore, thereby enhancing correct predictions while suppressing wrong predictions.

% This reveals significant headroom when improving the top-1 accuracy of multi-modal models. 
% %
% Our analysis has revealed several interesting findings for why top-1 accuracy is low in zero-shot settings. 
% %
% Closing the gap between top-1 accuracy and top-5 is under-explored.
% %
% This is particularly promising in multi-modal models compared to traditional supervised approaches as the proposed method can
% \begin{compactitem}
% \item allow easy ensembling over queries / prompts in their shared latent space, as different prompts yield different outputs [3,4].
% \item easily leverage hierarchy of class labels due to the multi-modal nature.
% \end{compactitem}
% %
% We note that the proposed post-processing techniques are simple and can be applied to any multi-modal models. 
% %
% Our experiments show 16.97\% improvement on the top-1 accuracy (21.63\% to 37.60\%) for the low confidence samples, and overall 3.6\% on the top-1 accuracy (64.18\% to 67.78\%) for all samples in ImageNet. 
% %
% %MH: the following sentences can be moved to conclusion (no need to discuss future work at the end of first section).
% %These results can be improved further.  
% %
% %Improving top-1 accuracy is known to improve calibration, robustness and out-of-distribution detection ( see plex-paper). 
% %
% %We plan to evaluate how the proposed technique improves uncertainty and robustness. 


% We make two main contributions in this work. 
% %
% First, we proposed a simple yet very effective prompt engineering method by using hierarchical label tree to improve zero-shot classification performance.
% %
% Second, the proposed method is tuning-free and parameter-free, and is applicable to re-rank any initial prediction ranking lists of image-text models.  



%%%%%%%%%%%%%%
%%%%%%%%%%%%%% related works
%%%%%%%%%%%%%%

\section{Related work}
% \vspace{-0.5em}
% \paragraph{Prompt engineering and learning}
% Our re-ranking method essentially leverages the rich label hierarchy to craft the prompts, therefore is related to prompt engineering.
%

%\paragraph{Confidence estimation} 
\noindent \textbf{Confidence estimation.} Reliably estimating the confidence of a prediction is helpful for downstream decision making and can ensure the safe deployment of machine learning models. A well-calibrated confidence estimation should assign low scores for incorrect predictions and high score for correct predictions.
Maximum softmax probability \cite{hendrycks2016baseline} and maximum logit \cite{hendrycks2019scaling} are the most commonly used confidence scores for classification problems, because of their simplicity and computational efficiency. 
Recent works propose more sophisticated confidence estimation methods which either involve modifications to the classification models or significantly increase the inference time. For example,
Bayesian approaches such as Gaussian Process layer \cite{liu2022simple} and dropout-based variational inference \cite{gal2015dropout} assume the weights in the neural networks are random variables such that the final prediction follows a distribution. A large variance of a prediction indicates the low confidence of the prediction. 
Non-Bayesian methods such as ensemble-based methods which aggregate the predictions from multiple models to improve the robustness of the confidence estimation \cite{Lakshminarayanan2017, wen2020batchensemble}. 
Those sophisticated methods were developed and studied in the single-modal models, and the application to multi-modal models is not straightforward. In addition, those methods mostly require modification to the model and additional training, which becomes challenging to multi-modal models since the training data are generally not publicly available. 
In our work, we focus on a zero-shot confidence estimation that is exclusively designed for multi-modal models. 
Our method does not require additional training, and is simple, efficient, and effective. 

%\paragraph{Prompt engineering}
\noindent \textbf{Prompt engineering.}
Prompt engineering and learning has attracted much attention in vision and learning since the introduction of image-text models \cite{radford2021learning, jia2021scaling, zhai2022lit}. 
%
The image-text models align images and their text descriptions into a common space, which facilitates model generalization to unseen categories at inference time. 
%
However, it has been observed that downstream image classification accuracy highly depends on the specific input prompts. 
%
This motivates researchers to either fine-tune or auto-learn prompts when adapting multi-modal models to downstream vision tasks.
\cite{zhou2022learning, zhou2022conditional} propose CoOp and CoCoOp to automatically learn the prompt word embeddings in the few-shot settings, and show significant improvements over the vanilla zero-shot image classification based-on prompting. 
%
%MH: learning? or supervised?
These are learning based approaches, requiring supervised data from downstream tasks, while our proposed method is zero-shot and post-hoc without using any supervised data. 
%
% In contrast, \citet{radford2021learning} suggest different approaches for prompt engineering.
% %
% %MH: I do not understand this sentence 
% For generic object and scenes, using template ``a photo of \{class\}''; for fine-grained categorization, type related context is added, e.g., ``a type of food'' for Food101. All the suggested crafting only changes the context, but fix the ``class'' in the template. Our method is different from them in that we fix the context, but only adapt the ``class''.
In concurrent work, \cite{shu2022test} proposes learning prompt embeddings in an unsupervised manner by minimizing the entropy of the averaged prediction probability distribution, where each prediction is based on a random augmentation applied to the input image.
Our work differs from \cite{shu2022test} in the sense that we do not learn an input-dependent prompt embedding. Instead we only selectively modify the prompts using knowledge hierarchy for images that have unreliable predictions, and our modified new prompt is natural language rather than a numerical embedding. 

%\paragraph{Label hierarchy}
\noindent \textbf{Label hierarchy.}
Label hierarchy or label ontology are relational graphs among semantic labels. WordNet is one of the most widely used concept ontologies, and it has been used for visual recognition problems. Fergus et al. \cite{fergus2010semantic} leverage the
WordNet hierarchy to define a semantic distance between any two categories and use this semantic distance to share labels. Deng et al. \cite{deng2014large} propose a hierarchy and exclusion graph to explicitly model the semantic relations among labels, and significantly improve object classification by exploiting the rich label hierarchy. The idea of semantic distance defined on the WordNet ontology graph is also used in \cite{rohrbach2011evaluating,rohrbach2010helps} for transferring knowledge in zero-shot learning problems. We are similar to the above work in that we utilize the label semantics encoded by the label hierarchy as well, but label hierarchy in our case is used in the multi-modality scenarios: textual labels and visual images are represented in the same latent space, therefore, the hierarchy structure is directly exploited in the representation space to steer the recognition process.  

% \paragraph{Re-ranking} 
% \todo{Is the connection between re-ranking and our method that we add children nodes to the ranking list which is regarded as ``expanding the neighbor list''? if so, can we make this clear at the begining of this paragraph?}
% Re-ranking is widely studied in text and image retrieval communities, and is mainly designed as a post-processing step to reorder an initial ranked lists, with the expectation that the close matches receive high ranks.
% %
% Here we review the related re-ranking vision approaches for object retrieval.  

% Given an initial $k$-nearest neighbors, existing methods typically expand the query or expand the neighbor lists for the re-ranking.
% \todo{not sure if the following is relevant to our work}
% For example,  \citet{chum2007total} uses the average of the kNN results as the new query to re-query the database and 
% \citet{shen2012object} take each image in the initial kNN list as a new query to produce a full $k \times k$ NN list, and recompute scores of each image based on its location in the $k \times k$ list. 
% %
% The concept of k-reciprocal nearest neighbors is adopted in \cite{qin2011hello,zhong2017re} to remove potential false matches in an initial ranking list. 
% %
% Our work is different from all the above-mentioned schemes in that we handle re-ranking in the multi-modality space, while all the above works are in the single vision embedding space.
  


%%%%%%%%%%%
%%%%%%%%%%%
%%%%%%%%%%% Section 2 Zero-shot failure case analysis
%%%%%%%%%%%
%%%%%%%%%%%





%%%%%%%%%%%
%%%%%%%%%%%
%%%%%%%%%%% Section 3 Zero-shot failure case analysis
%%%%%%%%%%%
%%%%%%%%%%%
% \vspace{-1.5em}
\section{Zero-shot inference failure case analysis}
\label{sec:failure_analysis}
% \vspace{-1em}

%%%%%%%%%%%
%%%%%%%%%%% Figure-1  
%%%%%%%%%%%

% \begin{figure}[tp]
% \centering
% \caption{Overview of top-5 correct, but top-1 incorrect classes in ImageNet}
% \includegraphics[width=\textwidth]{fig/Fig-failure-overall.png}
% \label{fig:failure}
% \end{figure}


Given that the top-1  accuracy (64.2\%) is much lower than top-5 accuracy (89.4\%) for zero-shot ImageNet classification using CLIP, we investigated the failure cases that are ``top-5 correct but top-1 wrong" (12605 images, 25.2\% of all test images). Table.~\ref{tab:freq_class_top1_wrong} in appendix shows some representative classes.
% The most frequent ground-truth classes those images belong to are shown in Table~\ref{tab:freq_class_top1_wrong}. %From the investigation, we revealed several failure modes as follows.  
The failure modes are summarized as:



\noindent{\bf (1) Class name does not specify super-class name: }% Model scores being affected by choice of words in class names
% \todo{make it consistent with figure title}: 
Some classes, whose class names do not have their WordNet ancestor (e.g., ``tusker", one of 1k ImageNet classes, does not have its parent ``elephant" in the class name), may have a relatively lower score than other classes, which explicitly have the ancestor present in the class name (e.g., ``Asian elephant'').
See examples in Fig.~\ref{fig:failure-mode} (Left).\\ 
% We observed that 47 of 50 tusker images are wrongly classified as other fine-grained elephant classes. That is because the ``tusker'' class name does not explicitly show that it belongs to elephant class, resulting in ``tusker" word embedding is not close to the image embedding. Similar mistakes happened for ``Collie": 45 of 50 collie images are wrongly classified by CLIP. We find most of them are wrongly classified as Shetland Sheepdog, which explicitly include the dog super class, while collie only implicitly indicate the dog class. Interestingly, we find adding the ``dog'' word concatenated with original class fix all the errors, which verified our assumption.
%%%%%%%%%%%
%%%%%%%%%%% Figure-2  failure-mode-1
%%%%%%%%%%%
% \begin{figure}[tp]
% \centering
% \includegraphics[width=\textwidth]{fig/Fig-fail-mode-1.png}
% \caption{Failure mode 1: Explicit or implicit show the super class, model scores being affected by choice of words in class names}
% \label{fig:failure-mode-1}
% \end{figure}
\noindent{\bf (2) Class name does not  specify sub-class name}: If the class name is too abstract, then its CLIP embedding is not necessarily close to the image embedding: e.g, CLIP wrongly classifies most images from ``balloon'' class as airship, see Fig.~\ref{fig:failure-mode} (Middle). That is because there are distinct kinds of balloons, each belonging to a different semantic subgroup. Relying on the text embedding of the fine-grained children's class names (e.g., using ``hot-air balloon'') often fixes these errors. \cite{beyer2020we} reported the similar issue of label ambiguity in ImageNet. \\
%%%%%%%%%%%
%%%%%%%%%%% Figure-3  failure-mode-2
%%%%%%%%%%%
% \begin{figure}[tp]
% \centering
% \includegraphics[width=\textwidth]{fig/Fig-fail-mode-2.png}
% \caption{Failure mode 2: Ambiguity words}
% \label{fig:failure-mode-2}
% \end{figure}
\noindent{\bf (3) Inconsistent naming between class names: 
% Model’s inconsistent focus on adjective and noun
} Some ImageNet class names are nouns, but  others are adjective-prefixed nouns. This may make CLIP text embedding biased, see one example in Fig.~\ref{fig:failure-mode} (Right) where images from ``screw'' class are misclassified as ``metal nail''.

% As observed from the failure modes (more examples shown in Appendix \ref{fig:qualitative-result}), many prediction mistakes could be fixed by using label relations: label hierarchy is not explicitly enforced in the training time of CLIP, then in the downstream object classification tasks, it could lead to predictions that violate the real world semantics: e.g., a ``doberman'' image could have a higher similarity with the word ``cat'' than ``dog'', although a object classified as ``doberman'' is automatically a ``dog'' as well. Since label hierarchical semantics are not modeled in the training time, this motivates us to explicitly employ label hierarchy (i.e., WordNet) in the inference time as a remedy to guide the classification process by ruling out prediction inconsistencies.   

%%%%%%%%%%%
%%%%%%%%%%% Figure-4  failure-mode-3
%%%%%%%%%%%

% \begin{figure}[tp]
% \centering
% \includegraphics[width=\textwidth]{fig/Fig-fail-mode-3.png}
% \caption{Failure mode 3: Inconsistent focus on adjective and noun
% }
% \label{fig:failure-mode-3}
% \end{figure}


% \noindent{\bf (4) Model score does not follow / reflect WordNet hierarchy}, which mismatch with human prior knowledge. For example, as shown in Fig.~\ref{fig:failure-mode}(4), the score for “dog” is not higher than the score for  “doberman”. \todo{our method does not fix this issue, maybe remove}

%%%%%%%%%%%
%%%%%%%%%%% Figure-5  failure-mode-4
%%%%%%%%%%%

% \begin{figure}[tp]
% \centering
% \includegraphics[width=0.6\textwidth]{fig/Fig-fail-mode-4.png}
% \caption{Failure mode 4: Inconsistent focus on adjective and noun \todo{increase the resolution or remove}
% }
% \label{fig:failure-mode-4}
% \end{figure}

% \noindent{\bf (5) The model has bias and different sensitivity to different words}, which may be caused by different words having different frequencies (potentially long-tail) during CLIP training. \todo{our method does not fix this issue, maybe remove}

% \noindent{\bf Key conclusions:} (1) Zero-shot inference (word embedding) is unstable and sensitive to words used in prompts.
% (2) ImageNet class names, having different intra-class variances, located at different level of WordNet and having inconsistent meaning, may not be sufficient to represent human's knowledge to the class, which cause the unstable and low performance on top 1.
% \vspace{-10pt}

\begin{figure*}[t]
% \vspace{-10pt}
\centering
%\includegraphics[width=\textwidth]{fig/Fig-hierarchy.pdf}
%  \includegraphics[width=\textwidth]{fig/zero-shot-figure-updated.pdf}
%  \includegraphics[width=\textwidth]{fig/zero-shot figure.pdf}
 \includegraphics[width=\textwidth]{zero_shot_figure.pdf}
%\includegraphics[width=\textwidth]{fig/Fig-method.pdf}
% \vspace{-1em}
\caption{ Our zero-shot classification pipeline consists of 2 steps: confidence estimation via self-consistency (left block) and top-down and bottom-up label augmentation using the WordNet hierarchy (right block). See
Algorithms~\ref{alg:uncertainty} and \ref{alg:hierarchy} %in Appendix~\ref{app:algorithm} 
for pseudocode.
}
\label{fig:method}
% \vspace{-2em}
\end{figure*}
% \vspace{-1em}

\section{Proposed Method}
% \vspace{-10pt}
%\section{Zero-shot uncertainty estimation} \label{sec:method_uncertainty}

As shown in Section \ref{sec:failure_analysis}, CLIP models can be sensitive to different text prompts for images in certain classes. 
% One cause could be some class names are ambiguous.
% Another possible cause could be that some classes have show less frequently (potentially long-tail) during CLIP training so that their text embeddings can be easily affected by data from other major classes during gradient descent, i.e. a less meaningful and robust. 
% For example, the class `fig` has the highest mean cosine similarity score, while the class `desert grassland whiptail lizard` has the smallest mean cosine similarity score. 
In this section, we first propose a confidence estimation method to identify low confidence predictions. 
We show that the identified subset has much lower accuracy than the average (Sec.\ref{sec:confidence_estimation}).  
% In the next section \ref{sec:method_hierachy}, 
We next develop a principled method that utilizes knowledge hierarchy to improve the accuracy of the low confidence subset, and consequently improve the overall accuracy on the whole datasets (Sec.~\ref{sec:method_hierachy}).  
% \vspace{-1em}
%\subsection{Zero-shot confidence estimation via self-consistency}
\subsection{Self-consistent zero-shot confidence estimation}
\label{sec:confidence_estimation}
% Word prompts need to be better calibrated such that they can be fairly compared in the ranking. We also leverage this finding to sparsify the WordNet hierarchy by removing rare words and to better make use of WordNet hierarchy.
Given an image $\vx$ and a candidate class name $c$, where $c\in \mathcal{C}, |\mathcal{C}|=1000$, the CLIP model encodes $\vx$ and $c$  respectively by its image encoder $f_{image}$ and text encoder $f_{text}$, denoted as $\vz_m=f_{image}(\vx)$ and $\vz_c=f_{text}(c)$. 
The prediction logit score is  defined as $\text{logit}(\vx, c) = \cos(\vz_m, \vz_c)$,  where $\cos(\cdot, \cdot)$ is the cosine similarity between two vectors, and the predicted class is $\argmax_{c\in\mathcal{C}} \text{logit}(\vx, c)$.
% To estimate the confidence of the prediction $\text{logit}$,
We estimate the confidence by the self-consistency rate when applying different context prompts and image augmentations. %respectively.
% $\vz_m$ or $\vz_c$, respectively.
% \vspace{-1em}

\paragraph{Confidence estimation via text prompts.}
% \noindent \textbf{Confidence estimation via text prompts.}
% We detect the low confidence subset based on the prediction's self-consistency to prompts. 
To improve the zero-shot classifier's performance, the CLIP paper \citep{radford2021learning} hand crafted various context prompts, e.g. ``\texttt{A photo of a big \{label\}}'' and ``\texttt{A photo of a small \{label}\}''), for different datasets for the purpose of prompt ensembling: 
For an image $\vx$, given a set of context prompts $\mathcal{T}$, the ensembled logit score is $\text{logit}(\vx, \mathcal{T}(c))=\frac{1}{|\mathcal{T}|}\sum_{t\in\mathcal{T}} \text{logit}(\vx, t(c))$, where $t(c)$ denotes the new prompt after applying context prompt $t(\cdot)$ to $c$. 
Here instead of using the prompts for ensembling, we make use of the prompts to define our confidence score. 
Given a set of prompts $\mathcal{T}$, we apply each of the prompt $t(\cdot)$ for the classifier, and see if the top-1 prediction is the same as that when applying no prompt. 
We use the percentage of prompts that have consistent top-1 prediction with that without prompt as the confidence score $S_{\mathcal{T}}(\vx)$, i.e.
\begin{align}
    S_{\mathcal{T}}(\vx) = \frac{ \sum_{t\in\mathcal{T}} \mathbbm{1}\{ \hat{c}(\vx, t) = \hat{c}(\vx, \emptyset) \} }{|\mathcal{T}|}
    \label{eq:conf_prompt}
\end{align}
where $\hat{c}(\vx, \emptyset) = \argmax_{c \in \mathcal{C}}  \text{logit}(\vx, c)$ is the top-1 prediction using the pure class name, and $\hat{c}(\vx, t) = \argmax_{c \in \mathcal{C}} \text{logit}(\vx, t(c))$ is the top-1 prediction when applying prompt $t(\cdot)$.
% To estimate the confidence score, we partition the 80 prompts into $L\geq 2$ sets, get the predictions for the $L$ sets $\mathcal{T}_1$, $\mathcal{T}_2$ \ldots  $\mathcal{T}_L$, and see if the top-1 prediction classes are the same or not.
Intuitively, a reliable prediction should have highly consistent top-1 predictions when context prompts are applied or not, and therefore should have a high confidence score $S_{\mathcal{T}}(\vx)$ with respect to the prompt set $\mathcal{T}$, and vice versa. 
% that no matter what the class-agnostic context prompt is applied, 
% To see if the prediction is robust, we apply two different set of context prompts $\mathcal{T}_1$ and $\mathcal{T}_2$ to the class labels, and see if the top predicted classes are the same or not.
% Intuitively, a high reliable prediction should be the ones that no matter what the class-agnostic context prompt is applied, the rank of the predicted classes would be the nearly the same.
% Intuitively, a high reliable prediction should be the ones that no matter what the context prompt is applied, the rank of the predicted classes should be the nearly the same. By contrast, an unreliable prediction will be the ones where the ranking changes a lot when applying different context prompts.
% Thus we define a high confidence prediction only if the top-$1$ predicted class is consistent when $L$ different sets of context prompts $\mathcal{T}_1$, $\mathcal{T}_2$ ... $\mathcal{T}_L$ are applied, i.e. $\argmax_{c \in \mathcal{C}}\text{logit}(\vx, \mathcal{T}_1(c)) = \argmax_{c \in \mathcal{C}}\text{logit}(\vx, \mathcal{T}_2(c))$ = ... = $\argmax_{c \in \mathcal{C}}\text{logit}(\vx, \mathcal{T}_L(c))$. All other cases are considered as low confidence predictions.

% \todo{modify the pipeline based on the continuous methods}

% i.e. the set of top-$1$ predicted classes $\{c\in \mathcal{C}: |\{c' \in \mathcal{C}: \text{logit}(\vx_m, \mathcal{T}(c)) < \text{logit}(\vx_m, \mathcal{T}(c'))| < k \}$ are different when $\mathcal{T}=\mathcal{T}_1$ or $\mathcal{T}_2$. 
% We consider $k=5$ for common practice. 
% \begin{align*}
% \{t\in \mathcal{T}: |\{t' \in \mathcal{T}: \text{logit}(\vx_m, \mathcal{C}_1(\vx_t)) < \text{logit}(\vx_m, \mathcal{C}_1(\vx_{t'}))| < k \}
% %\neq \{t\in \mathcal{T}: |\{t' \in \mathcal{T}: \text{logit}(\vx_m, \mathcal{C}_2(\vx_t)) < \text{logit}(\vx_m, \mathcal{C}_2(\vx_{t'}))| < k \} 
% \end{align*}
%There can be different design choices for $\mathcal{T}$ and $L$. For simplicity, we use $L=2$ and the a random set of 40 context prompts in the list as $\mathcal{T}_1$ and the full 80 context prompts as $\mathcal{T}_2$. We studied other choices such as using a random set of 20 context prompts as $\mathcal{T}_1$, or using the first 40 context prompts in the list as $\mathcal{T}_1$, and found the results were very similar. 
% There can be different design choices for $\mathcal{T}_1$ and $\mathcal{T}_2$. For simplicity, we use the a random set of 40 context prompts in the list as $\mathcal{T}_1$ and the full 80 context prompts as $\mathcal{T}_2$. We studied other choices such as using a random set of 20 context prompts as $\mathcal{T}_1$, or using the first 40 context prompts in the list as $\mathcal{T}_1$, and found the results were very similar. 


% For each given image and candidate 1000 class labels, we use different prompt engineering method on the text embedding of class labels. Each kind of prompt engineering method will have their own decision for the given image. We select those images that with inconsistent decisions among different decision with different prompt engineering methods as the unstable images. 
% The assumption is that if CLIP model has high confidence for the given image, then no matter which kind of prompt engineering method we use, the decision should be same. If different prompts lead to different decision, then it indicates that CLIP has no enough confidence to make the decision given limited words to describe the class name.


\paragraph{Confidence estimation via image perturbation.} 
% \noindent \textbf{Confidence estimation via image perturbation.} 
We can also estimate the confidence of a prediction based on the self-consistency when applying different perturbations to the input image.
Intuitively, if the top-1 predictions are inconsistent when applying different image perturbations, the prediction is unreliable. 
Specifically, we consider the common image transformations, left-right flip, up-down flip, rotation, crop, etc., and apply the perturbation method $b(\cdot)$ to the input image, and infer the predicted class as $\hat{c}(\vx, b) = \argmax_{c\in \mathcal{C}}\text{logit}(b(\vx), c)$. 
We define the confidence score with respect to a set of image perturbations $\mathcal{B}$ as, 
\begin{align}
    S_{\mathcal{B}}(\vx) = \frac{ \sum_{b\in\mathcal{B}} \mathbbm{1}\{ \hat{c}(\vx, b) = \hat{c}(\vx, \emptyset) \} }{|\mathcal{B}|}
    \label{eq:conf_image}
\end{align}
% where $\hat{c}(\vx, b) = \argmax_{c \in \mathcal{C}} \text{logit}(b(\vx), c)$ is the top-1 prediction when applying prompt $t(\cdot)$.
We expect a high confidence prediction to have highly consistent prediction when applying different image perturbations, and therefore to have a high confidence score $S_{\mathcal{B}}(\vx)$ with respect to the image perturbation set $B$. 
% if the top-1 prediction of the perturbed image is inconsistent  with the raw image. 
% \todo{need to mention how we combine prompt ensembling and image perturbation. union of the two sets?}
% \todo{explain some perturbation works better than others.}
% For given image, we use different data augmentation methods that do not change the semantic meaning: left-right flip, up-down flip, rotation, crop, etc. Only those images, that has consistent decision among all different image augmentation method, are treated as high confidence image for CLIP. On the contrary, if the image has inconsistent decision after using different augmentation method, we select them as unstable image.
%%%%%
%%%%% Algorithm-1
%%%%%

\paragraph{Determining the low confidence subset by combining the two confidence estimations.}
% \noindent \textbf{Determining the low confidence subset by combining the two confidence estimations.}
The confidence score we proposed in Eq. (\ref{eq:conf_prompt}) and Eq. (\ref{eq:conf_image}) are continuous values. A threshold needs to be determined if we want to select a subset of examples with low confidence using the continuous confidence score. 
In practice, the threshold can be chosen based on the requirement of recall and precision trade-off in the real application.
In our study, to bypass the threshold selection, we propose to use a binary criterion for determining the low confidence set. 
% There can be different design choices for $\mathcal{T}_1$ and $\mathcal{T}_2$. For simplicity,

For IamgeNet dataset, the CLIP paper \cite{radford2021learning} designed total 80 context prompts. 
We define four sets based on the 80 prompts: the first 40 prompts $\mathcal{T}_1$, the last 40 prompts $\mathcal{T}_2$, all 80 prompts $\mathcal{T}_3$, and no prompts $\mathcal{T}_4=\emptyset$. 
We apply the four different sets of prompts to the classifier and see if their top-1 predictions are all consistent or not, i.e. $\hat{c}(\vx, \mathcal{T}_1) = \hat{c}(\vx, \mathcal{T}_2) = \hat{c}(\vx, \mathcal{T}_3) = \hat{c}(\vx, \mathcal{T}_4)$. 
Then we determine the low confidence subset $\mathcal{O}_\mathcal{T}$ as those examples who have inconsistent predictions among the 4 prompts sets.
% and the high confidence subset as those have consistent predictions vice versa.
% We use the a random set of 40 context prompts as $\mathcal{T}_1$ and the full 80 context prompts as $\mathcal{T}_2$.
We studied other choices such as using a random set of 40 prompts as $\mathcal{T}_1$, or splitting the 80 prompts into more subgroups, and found the results were very similar. 

Similarly we also determine a low confidence subset $\mathcal{O}_\mathcal{B}$ based on image perturbations. 
In practice we found left-right flip works the best among the above mentioned perturbations. 
Thus for simplicity, we compare the top-1 prediction when applying the left-right flip to the input image and the top-1 prediction when using raw image. If their predictions are not consistent, that example will be included into the low confidence set $\mathcal{O}_\mathcal{B}$. 

Finally, we use the union of the two low confidence sets $\mathcal{O}_\mathcal{T}$ identified using the text prompts and and $\mathcal{O}_\mathcal{B}$ identified using the image perturbations as the final low confidence subset $\mathcal{O}$ in the following
experiments. 
%
Algorithm \ref{alg:uncertainty} shows the low confidence set generation process. 



% 

\begin{algorithm}[tp]
\small
\caption{Zero-shot confidence estimation}
\label{alg:uncertainty}
%\begin{algorithmic}
% \definecolor{CommentColor}{HTML}{006619}
\SetKwInput{KwData}{Input}
\SetKwInput{KwResult}{Output}

\KwData{Input images $ \mathcal{X}=\{\vx_i\}_{i=1}^N$, Candidate class set $\mathcal{C}$, image encoder $f_{image}$ and text encoder $f_{text}$, text threshold $\tau_{t}$, image threshold $\tau_{i}$}
\KwResult{Low confidence set $\mathcal{O}$}
% , $L$ different context prompt $\{t_l\}_{l=1}^{L}$

\SetAlgoLined
%%%%%%%%
%%%%%%%% prompts
%%%%%%%%
\nl
Low confidence set $\mathcal{O}_{\mathcal{T}} \gets \emptyset$ \ \algcomment{Confidence estimation via text prompts}

\nl
Sample $L$ different context prompt $t_1$, $t_2$ \ldots  $t_L$

% \nl
% $\vz_m=f_{image}(\vx)$ and $\vz_c=f_c(c)$

\nl
\For{$\vx_i \in \mathcal{X}$}{
\nl
Compute $S_{\mathcal{T}}(\vx_i)$ based on Eq. (\ref{eq:conf_prompt})
% \nl
% \For{$t \in \{t_1$, $t_2$ \ldots  $t_L\}$}{
% \nl
% $\text{logit}(\vx_i, t(c)) \gets \cos(f_{image}(\vx_i), f_{text}(t(c)))$
% % \frac{1}{|\mathcal{T}|}\sum_{t\in\mathcal{T}} \textnormal{logit}(\vx_i, t(c))  \gets 

% }

\nl
\If { $S_{\mathcal{T}}(\vx_i)$ $>$ $\tau_{t}$}{
$\vx_i$ has  high confidence prediction
    }
\Else {$\mathcal{O}_{\mathcal{T}} \gets \mathcal{O}_{\mathcal{T}} \cup \vx_i$
}
}

%%%%%%%%
%%%%%%%% image perturbation
%%%%%%%%
\nl
Low confidence set $\mathcal{O}_{\mathcal{B}} \gets \emptyset$ \ \  \algcomment{Confidence estimation via  image perturbation}

\nl
Sample $M$ perturbation methods $b_1, \dots, b_M$ 

\nl
\For{$\vx_i \in \mathcal{X}$}{

Compute $S_{\mathcal{B}}(\vx_i)$ based on Eq. (\ref{eq:conf_image})

\nl
\If {$S_{\mathcal{B}}(\vx_i)$ $>$ $\tau_{i}$}{
$\vx_i$ has high confidence prediction
    }
\Else {$\mathcal{O}_{\mathcal{B}} \gets \mathcal{O}_{\mathcal{B}} \cup \vx_i$
}
}

\nl
$\mathcal{O} \gets \mathcal{O}_{\mathcal{T}} \cup \mathcal{O}_{\mathcal{B}}$
\end{algorithm}

% \begin{algorithm}[tp]
% \small
% \caption{Zero-shot confidence estimation}
% \label{alg:uncertainty}
% %\begin{algorithmic}
% % \definecolor{CommentColor}{HTML}{006619}
% \SetKwInput{KwData}{Input}
% \SetKwInput{KwResult}{Output}

% \KwData{Input images $ \mathcal{X}=\{\vx_i\}_{i=1}^N$, Candidate class set $\mathcal{C}$, image encoder $f_{image}$ and text encoder $f_{text}$}
% \KwResult{Low confidence set $\mathcal{O}$}
% % , $L$ different context prompt $\{t_l\}_{l=1}^{L}$

% \SetAlgoLined
% %%%%%%%%
% %%%%%%%% prompts
% %%%%%%%%
% \nl
% Low confidence set $\mathcal{O}_{\mathcal{T}} \gets \emptyset$ \ \algcomment{Confidence estimation via text prompts}

% \nl
% Sample $L$ different context prompt $t_1$, $t_2$ \ldots  $t_L$

% % \nl
% % $\vz_m=f_{image}(\vx)$ and $\vz_c=f_c(c)$

% \nl
% \For{$\vx_i \in \mathcal{X}$}{

% \nl
% \For{$t \in \{t_1$, $t_2$ \ldots  $t_L\}$}{
% \nl
% $\text{logit}(\vx_i, t(c)) \gets \cos(f_{image}(\vx_i), f_{text}(t(c)))$
% % \frac{1}{|\mathcal{T}|}\sum_{t\in\mathcal{T}} \textnormal{logit}(\vx_i, t(c))  \gets 

% }

% \nl
% \If {$\argmax_{c \in \mathcal{C}}\textnormal{logit}(\vx, t_1(c))$ = ... = $\argmax_{c \in \mathcal{C}}\textnormal{logit}(\vx_i, t_L(c))$}{
% $\vx_i$ prediction has high confidence
%     }
% \Else {$\mathcal{O}_{\mathcal{T}} \gets \mathcal{O}_{\mathcal{T}} \cup \vx_i$
% }
% }

% %%%%%%%%
% %%%%%%%% image perturbation
% %%%%%%%%
% \nl
% Low confidence set $\mathcal{O}_{\mathcal{B}} \gets \emptyset$ \ \  \algcomment{Confidence estimation via  image perturbation}

% \nl
% Sample $M$ perturbation methods $b_1, \dots, b_M$ 

% \nl
% \For{$\vx_i \in \mathcal{X}$}{

% \nl
% \For{$b \in \{b_1$, $b_2$ \ldots  $b_M\}$}{
% \nl
% $\textnormal{logit}(b(\vx_i), c) \gets \cos(f_{image}(b(\vx_i)), f_{text}(c))$
% }

% \nl
% \If {$\argmax_{c \in \mathcal{C}}\textnormal{logit}(b_1(\vx_i), c)$ = ... = $\argmax_{c \in \mathcal{C}}\textnormal{logit}(b_M(\vx_i), c)$}{
% $\vx_i$ prediction has high confidence
%     }
% \Else {$\mathcal{O}_{\mathcal{B}} \gets \mathcal{O}_{\mathcal{B}} \cup \vx_i$
% }
% }

% \nl
% $\mathcal{O} \gets \mathcal{O}_{\mathcal{T}} \cup \mathcal{O}_{\mathcal{B}}$
% \end{algorithm}






%%%%%%%%%%%
%%%%%%%%%%% Section Top-down and bottom-up classification with knowledge hierarchy
%%%%%%%%%%%
% \vspace{-1em}
\subsection{Top-down and bottom-up label augmentation using WordNet hierarchy}
\label{sec:method_hierachy}
%\section{Top-down and bottom-up class name augmentation using WordNet hierarchy} \label{sec:method_hierachy}
%%%%%%%%%%%
%%%%%%%%%%% Figure-6  Hierarchy method
%%%%%%%%%%%
Through extensive %investigations 
analysis of the incorrect predictions among the identified unreliable predictions, we %noticed
found that many of them are caused by CLIP's lack of robustness to prompts. Instead of tuning the prompt templates, we focus on how to augment {\small\texttt{\{label\}}} in ``{\small\texttt{A photo of a \{label\}}}''. 
A proper prompt that specifies both the generic type and the more specific sub-types of this class are very important for correctly classifying the image.
However, the ImageNet class names are not all defined with similar specificity and some classes are more abstract than others, e.g. 350 classes have children, while the rest of the classes have no children. See appendix Fig.~\ref{fig:hierarchy} for more details. 
% shows the hierarchy statistics . 
% We looked up the 1000 ImageNet class names in WordNet hierarchy and found that they are not in the same level. There are 350 classes are at higher levels of the hierarchy with children, while other classes 650 classes are at the bottom of the hierarchy with no children. The number of children also vary a lot. The statistics are shown in Figure \ref{fig:hierarchy}(b).
To make the ImageNet classification problem better suited to CLIP, we leverage the underlying WordNet hierarchy and develop a top-down and bottom-up class name augmentation method to improve zero-shot prediction accuracy for unreliable predictions.
% \vspace{-1em}


The WordNet hierarchy is a semantic concept ontology, with nodes being cognitive synonyms indicating different concepts, and edges indicating the super-subordinate relation between concepts. Traveling upward from edges to the root, the concepts start from the very specific to the generic. 
For example, starting from the edge node ``strawberry'' to the root are ``berry'',  ``edible fruit'', ``produce'', ``food'', ``solid'', ``matter'', and ``physical entity'' (the root).
% The ancestors of the edge node ``jellyfish''  are ``coelenterate'', ``invertebrate'', ``animal'', ``organism'', ``living thing'', ``whole, unit'', ``object'', and ``physical entity'' (the root).
As we have seen in the failure mode analysis, many of the imageNet class names suffer from either being too abstract or being too specific, so that their concepts do not align well with the visual concepts the CLIP model learned in training. We propose using the WordNet knowledge hierarchy to augment the class labels in prompts so that the CLIP model has a better match between the image and prompts. 
% Label semantic relations from WordNet hierarchy are explored in the single-modality visual recognition work \cite{deng2014large,fergus2010semantic} to regularize the training process, while they are not modeled in CLIP's objectives, 
% we propose to use WordNet label hierarchy to re-calibrate the logit score between image and the corresponding label in the inference time.

\paragraph{Top-down: augmenting class names with parent.}
% \noindent \textbf{Top-down: augmenting class names with parent.}
As shown in failure case analysis, adding the super-class name to reduce ambiguity and to encourage the model's attention on the generic concept is helpful for improving the accuracy. 
Therefore we propose using WordNet to find the parent node of the raw class name, and concatenate it to the class name, i.e.
%\begin{align*}
$
    \text{logit}(\vx, c) = \text{logit}(\vx, [c; p(c)])
$
%\end{align*}
where $p(c)$ is the parent node's name of the class name $c$, and $[c; p(c)]$ means the string concatenation of the class name and the parent name.
We apply the method to top-5 predicted classes. Using the newly defined class names, we are able to re-rank the top-5 predictions for the identified unreliable subset of images. 
Note that WordNet contains a few very abstract class names for nodes, such as ``physical entity'', ``artifact'', ``matter'', etc. 
We found that such parent nodes are not informative, hence we remove them.
There are also many academic words in WordNet, for example the parent node of sea anemone is ``anthozoan'',
%actinozoan
 which can be rare in CLIP training data. 
Adding those academic words to class name makes the prediction even less robust. 
So we simplify the WordNet by pruning based on an estimation of the word frequency in CLIP training data by using embedding norm. 
%See Appendix~\ref{sec:sparse_wordnet} for more details. 

% Inspired by these findings, we investigated several techniques to improve top-1:
% Using WordNet hierarchy to improve the zero-shot inference, we use both top-down and bottom-up strategies.
%Top-down: we add the lowest common ancestor (LCA) with the ImageNet word label to perform as attention during inference, and help CLIP utilize the context information to make the final decision (re-ordering the top 5)


% \vspace{-1em}
\paragraph{Bottom-up: augmenting class names with children.}
% \noindent \textbf{Bottom-up: augmenting class names with children.}
Some ImageNet class names are generally abstract, but the ImageNet images may belong to a specific subtype of the class. For example, ``balloon'' is a class name in ImageNet, but most balloon images in ImageNet are actually ``hot-air balloon'', which is a child of ``balloon'' in WordNet hierarchy. The logit score for a parent class is not necessarily higher than the score for its child classes, mismatching with hierarchy prior. To accurately classify the images using CLIP, we need to augment the class name with fine-grained child subclasses. 
For each class $c$ having children in the WordNet hierarchy, we redefine the logit score as the max score over itself and all its children, i.e.,
%\begin{align*}
$
    \text{logit}(\vx, c) = \max \{\text{logit}(\vx, c), \text{logit}(\vx, c_1), \dots, \text{logit}(\vx, c_r)\},
$
%\end{align*}
where $c_1 \dots c_r$ are the $r$ children of the node $c$ in the WordNet hierarchy. 
We apply this bottom-up method to top-$5$ predicted class names, and re-rank the top predictions. 

% \noindent \textbf{Combining Top-down and bottom-up.}
\paragraph{Combining Top-down and bottom-up.}
In practice, we use both children and the ancestor to augment each class $c$, to transfer semantic information bidirectionally in both top-down and bottom-up way: the ancestor class is more generic than $c$, and has better chance to disambiguate instance from a more abstract level; on the other hand, children categories have more specific attribute description, and the attribute descriptions are semantically meaningful representations bridging the gap between the image embedding and its abstract class concept $c$. Then the final logit score between $x$ and $c$ is: 
\begin{multline}
    \text{logit}(\vx, c) =\max \{\text{logit}(\vx, [c; p(c)]), \\ \text{logit}(\vx, [c_1; p(c)]), \dots, \text{logit}(\vx, [c_r; p(c)])\}
    \label{eq:logit_tp_bu}
\end{multline}
where $p(c)$ is parent of $c$, and $c_1 \dots c_r$ are $c$'s children. The $\hat{c}$, where $\hat{c}\in \mathcal{C}_{top5}$, with the maximal logit score is the predicted class of $\vx$. 
%
See Algorithm \ref{alg:hierarchy} for details.


%%%%%%%%
%%%%%%%% Algorithm-2
%%%%%%%%
\begin{algorithm}[tp]
\small
\caption{Top-down and bottom-up class label augmentation using WordNet hierarchy}
\label{alg:hierarchy}
%\begin{algorithmic}
% \definecolor{CommentColor}{HTML}{006619}
\SetKwInput{KwData}{Input}
\SetKwInput{KwResult}{Output}

\KwData{Input image $\vx \in \mathcal{O}$, top-5 candidate class set $\mathcal{C}_{top5}$, sparse WordNet hierarchy $H$, image encoder $f_{image}$ and text encoder $f_{text}$}
\KwResult{Predicted class of $\vx$}

\SetAlgoLined

\nl
Candidate class set $\mathcal{C} \gets \emptyset$ 

\nl
\For{$c \in \mathcal{C}_{top5}$}{

$\mathcal{C} \gets \mathcal{C} \cup [c; \textnormal{parent}(c)]$, where $\textnormal{parent}(c)$ is the parent of $c$ in $H$
\ \  \algcomment{Top-down}

\nl
\If{$c$ \textnormal{has} $r \geq 1$ \textnormal{children} $c_1 \dots c_r$ in H }{
$\mathcal{C} \gets \mathcal{C} \cup \{[c_j; \textnormal{parent}(c)]\}^{r}_{j=1}$ \ \  \algcomment{Bottom-up}
}
}

\nl
$\hat{c} \gets \argmax_{c \in \mathcal{C}} \textnormal{logit}(\vx, c)$

\If{$\hat{c}\in \mathcal{C}_{top5}$}{ final prediction $\gets \hat{c}$ }
\Else {final prediction $\gets \textnormal{parent}(\hat{c})$}
%  where $p(\hat{c}) \in \mathcal{C}_{top5}$
\end{algorithm}




\paragraph{Sparsifying WordNet using the norm of text embeddings.} 
%\label{sec:sparse_wordnet}
% \vspace{-0.5em}
WordNet contains many academic words that are rarely used in common usage of English, and hence unlikely to occur frequently in the captions used for CLIP training. For example, ``anthozoan, actinozoan'', ``coelenterate'', ``gastropod'', and etc..
Directly using the raw WordNet with academic words as parents is not helpful for improving zero-shot accuracy, and can even harm the performance. 
Though we do not have access to the CLIP private data, we study the norm of the word embedding vector and found it is correlated with word frequency. 
We compute the $L_2$ norm of the word embedding when the word is coupled with different context prompts, i.e., $\rVert f_{text}(t(c)) \rVert$, $t \in \mathcal{T}$. 
We found that the variance of the norm, $\Var_{t\in\mathcal{T}}(\rVert f_{text}(t(c)) \rVert)$, is correlated with word frequency. Rare words tend to have small variances, while common words tend to have large variances. 
For example, the variance of the rare word ``anthozoan'' is 0.118, while the variance of the more common words 
``workplace, work'' is  0.724. 
We use this statistic to filter out rare words in WordNet. We removed 60\% of the nodes in WordNet and only kept the top 40\% nodes with the highest variance.
Our intuition behind the correlation between the norm variance and the word frequency is that, for a frequent word that has many examples in the CLIP training data, the CLIP model learns a very precise text embedding such that it has the capability to tell the semantic difference under different contexts, e.g., ``{\small\texttt{a photo of a nice \{label\}}}'' and ``{\small\texttt{a photo of a weird \{label\}}}''. 

% \todo{add examples what we filtered}


% % 'a photo of a nice {}.',
% %  'a photo of a weird {}.',
% % 'a bad photo of a {}.',
% %  'a photo of many {}.',
% %  'a sculpture of a {}.',
% %  'a photo of the hard to see {}.'
% % ``\texttt{a good photo of the {label}.}''
% % 'a blurry photo of the {}.',

% \vspace{-1em}
\section{Experiments and Results}
% \vspace{-1em}
Our proposed method is composed of two steps and we conduct experiments to verify the effectiveness of each step: 
(1) Use zero-shot confidence estimation to identify the low confidence subset of samples (see Fig.~\ref{fig:conf_esti} for the results), and
(2) Augment the class label using top-down and bottom-up strategies based on the sparsified WordNet on the low confidence subset to improve the accuracy (See Table~\ref{table:zero-shot} for the results).
%%%%%%%
%%%%%%% Fig- selective prediction
%%%%%%%
% \begin{wrapfigure}{r}{0.45\textwidth}

\begin{figure*}[htb]
\centering
\begin{subfigure}[t]{0.35\textwidth} % changed for arxiv
\centering
\caption{CLIP: Calibration ROC and AUC}
\vspace{-1.5em}
\includegraphics[width=0.96\textwidth]{clip_auc.pdf}
\label{fig:clip_auc}
\end{subfigure} 
\begin{subfigure}[t]{0.35\textwidth} % changed for arxiv
\centering
% \vspace{-0.05em}
\caption{CLIP: Selective prediction}
\includegraphics[width=0.84\textwidth]{clip_selective_pred.pdf} 
\label{fig:clip_sp}
\end{subfigure} 
% \vspace{0.5em}
% \vspace{0.5em}
% \vspace{-1.5em}
\begin{subfigure}[t]{0.35\textwidth} % changed for arxiv
\centering
\caption{LiT: Calibration ROC and AUC}
\includegraphics[width=0.84\textwidth]{lit_auc.pdf}
\label{fig:lit_auc}
\end{subfigure} 
\begin{subfigure}[t]{0.35\textwidth} % changed for arxiv
\centering
% \vspace{-15pt}
\caption{LiT: Selective Prediction}
\includegraphics[width=0.84\textwidth]{lit_selective_pred.pdf} 
\label{fig:lit_sp}
\end{subfigure} 
% \vspace{-0.1em}
% \vspace{0.8em}
\caption{ROC plots (left column) show that our proposed confidence score is better at distinguishing correct and incorrect predictions and results in higher AUC scores than baselines for both CLIP (ViT-B/16) (a) and LiT (ViT-B/32)(c). Selective prediction curves (right column) show that our proposed confidence score is better at abstaining incorrect predictions and as a result the accuracy of the remaining set is higher than the baselines for both CLIP (ViT-B/16) (b) and LiT (ViT-B/32) (d). }
\label{fig:conf_esti}
\end{figure*}

% \begin{figure*}[htb]
% \centering
% %  \vspace{-1em}
% % \includegraphics[width=0.45\textwidth]{fig/Fig-select-pred-result.pdf}
% % \includegraphics[width=.8\textwidth]{fig/selective prediction all-2.pdf}
% \includegraphics[width=.8\textwidth]{fig/fig-3-all.pdf}
% %  \vspace{-1.5em}
% \caption{Selective prediction accuracy at different abstention rates for (a) CLIP model and (b) LiT model. \todo{please add more details to the captions, e.g, what these 4 plot mean?}
% % See Figure~\ref{fig:select-pred-result-LiT} in Appendix~\ref{app:additional:results} for similar results on LiT.  
% %Our proposed confidence estimation is better suited for CLIP on selecting the correctly predicted set than the logit-based method (consistently improve around 7\% on top-1 zero-shot accuracy).
% }
% % \todo{add figure for LiT}
% % (b) The proposed combined quality score based on OOD scores and Perplexity that predicts output quality (rouge, bleu, huamn eval etc.) better than individual scores. \todo{Put figures next to each other?}
% \label{fig:select-pred-result}
% \end{figure*}
% % \vspace{-0.5em}
% % \end{wrapfigure}


% %%%%%%%
% %%%%%%% Fig- selective prediction density
% %%%%%%%
% \begin{figure*}[htb]
% \centering
% \includegraphics[width=.8\textwidth]{fig/density.pdf}
% \caption{Selective prediction density with different confidence score. 
% }
% \label{fig:select-pred-density}
% \end{figure*}




\begin{table*}[tp]
\large
%   \footnotesize
% \scriptsize
\centering
% \vspace{-5pt}
\caption{CLIP (ViT-B/16) and LiT (ViT-B/32) zero-shot top-1 accuracy comparison between baseline and ours (w/ hierarchy).}
%\rowcolors{2}{gray!25}{white}
\scalebox{.7}{%
\begin{tabular}{l c |c c| c c}
    \toprule
 %   \rowcolor{LightCyan}
     & & CLIP & (Ours) Hierarchy-CLIP & LiT & (Ours) Hierarchy-LiT\\
    % iamgenet
    \midrule
     \multirow{2}{*}{ImageNet} & Low conf. set  & 21.58\% & \bf{38.71\%}  & 31.18\% & \bf{37.25\%} \\ 
     & Full set & 64.18\% & \bf{67.78\% } & 68.26\% & \bf{69.41\% }  \\ 
 % \multirow{2}{*}{ImageNet} & Low confidence subset (9340) 

     
     % iamgenet-v2
    \midrule
 %   \rowcolor{Gray}
     \multirow{2}{*}{ImageNet-v2}& Low conf. set  & 17.77\% & \bf{32.50\%} & 27.08\% & \bf{31.45\% }\\
 %    \rowcolor{Gray}
     & Full set  & 58.06\% & \bf{61.07\%} & 60.11\% & \bf{61.11\% } \\
    
    % iamgenet-R
    \midrule
     \multirow{2}{*}{ImageNet-R} & Low conf. set  & 16.79\% & \bf{27.91\% } & 21.82\% & \bf{22.93\% } \\
     & Full set & 56.88\% & \bf{59.46\%} & 66.54\% & \bf{66.75\% }  \\
    
    % iamgenet-Adversarial
    \midrule
 %  \rowcolor{Gray}
     \multirow{2}{*}{ImageNet-Adversarial} & Low conf. set  & 10.13\% & \bf{18.44\% } & 7.19\% & \bf{8.95\% }\\
     & Full set & 26.12\% & \bf{29.23\% } & 13.93\% & \bf{14.56\%}  \\
     
     % iamgenet-sketch
    \midrule
% \rowcolor{Gray}
     \multirow{2}{*}{ImageNet-Sketch} & Low conf set & 13.74\% & \bf{23.18\% } & 21.51\% & \bf{24.42\%}\\
     & Full set  & 44.71\% & \bf{47.28\% } & 52.47\% & \bf{53.17\% }  \\   
     
     \bottomrule
\end{tabular}
}
\label{table:zero-shot}
% \vspace{-12pt}
\end{table*}


\begin{table}[t]
% \large
%   \footnotesize
% \scriptsize
\centering
\vspace{-5pt}
\caption{CLIP (ViT-B-16) zero-shot top-1 accuracy comparison with prompt ensemble.}
\scalebox{0.65}{%
%\rowcolors{2}{gray!25}{white}
\begin{tabular}{l c |c c}
    \toprule
 %   \rowcolor{LightCyan}
     & & Ensemble only & Hierarchy and Ensemble \\
    % iamgenet
    \midrule
     \multirow{2}{*}{ImageNet} & Low conf. set  & 41.05\% & \bf{42.09\%}  \\ 
     & Full set & 68.48\% & \bf{68.86\% } \\ 
 % \multirow{2}{*}{ImageNet} & Low confidence subset (9340) 

     
     % iamgenet-v2
    \midrule
 %   \rowcolor{Gray}
     \multirow{2}{*}{ImageNet-v2}& Low conf. set  & \bf{36.39}\% &  36.34\% \\
 %    \rowcolor{Gray}
     & Full set  &   \bf{62.02\%} & 62.00\% \\
    
    % iamgenet-R
    \midrule
     \multirow{2}{*}{ImageNet-R} & Low conf. set  &  35.13\% & \bf{ 36.12\% }  \\
     & Full set &  60.21\% & \bf{ 60.62\%}   \\
    
    % iamgenet-Adversarial
    \midrule
 %  \rowcolor{Gray}
     \multirow{2}{*}{ImageNet-Adversarial} & Low conf. set  &  21.13\% & \bf{ 22.00\% } \\
     & Full set &  30.59\% & \bf{ 31.07\% }   \\
     
     % iamgenet-sketch
    \midrule
% \rowcolor{Gray}
     \multirow{2}{*}{ImageNet-Sketch} & Low conf. set &  \bf{27.13}\% &  26.56\% \\
     & Full set  &  \bf{48.52\%} & 48.26\%   \\   
     
     \bottomrule
\end{tabular}
}
\label{table:add_prompt}
% \vspace{-12pt}
\end{table}
% }



\subsection{Our proposed confidence score is better suited for selective prediction than baselines}
% .Confidence estimation for selective prediction}

A well-calibrated confidence estimator should score high for those correct predictions, and low for incorrect predictions. 
As a result, a good confidence estimator should be a good predictor for prediction correctness. We plot the receiver operating characteristic (ROC) curve and compute the area under the ROC curve (AUC) as a quantitative measure to compare our proposed confidence estimation with the baselines. 
An AUROC of 1.0 indicates perfect separation between correct and incorrect predictions, and 0.5 means the two groups are not distinguishable.
Maximum logit score, $\max_{c\in\mathcal{C}} \text{logit}(\vx, c)$ is one of the most commonly used confidence score for classification problems in single modal models \cite{hendrycks2019scaling}, so we consider it as our baseline. 
Fig. \ref{fig:clip_auc} and \ref{fig:lit_auc} clearly show that our confidence score is significantly better than the baseline method at distinguishing between correct and incorrect predictions, for both CLIP and LiT models. 
The AUC score for our proposed method is above 0.8 while that for the baseline method is around 0.7. 


We also compare our method with the baseline in the scenario of selective prediction.
Given a budget of abstention rate $\alpha\%$, the best strategy is to abstain the $\alpha\%$ samples with the lowest confidence scores. If the confidence score is well calibrated, the accuracy for the abstained set will be low and as an evidence the accuracy of the remaining set would be high.
We plot the selective prediction curves \citep{Lakshminarayanan2017}, which reports the accuracy on the remaining set as a function of the abstention rate. 
% We use each score to select the least confident 18\%, 21\%, and 27\% samples, and evaluate the accuracy on the remaining. Better confidence estimation allows model to better detect inputs where it is likely to be incorrect and abstain on such examples, as evidenced by the higher accuracy on the remaining set. 
Fig. \ref{fig:clip_sp} and \ref{fig:lit_sp} show that our proposed confidence score results in higher accuracy than the baseline maximum logit score at all abstention rates for both CLIP and LiT.

Prompt ensemble has been shown to improve accuracy and robustness of the prediction, so here we also compare ours with the maximum logit score after applying prompt ensemble. As shown in the selective prediction curves, although the prompt ensemble indeed helps to achieve higher accuracy (dashed line) than that using the pure class name (solid line), it is still inferior to our proposed method.
% \todo{did our proposed method also use prompt ensembles?}. 
% Thus \textit{our proposed confidence score is better suited for selective prediction than max logit baseline.} %-based confidence score.}
% At different confidence levels (low, medium, and high), we could select different subset of ImageNet by keeping only the image samples that has higher decision confidence score than the threshold (which shows that the model has enough confidence to make final decision, for those unconfident images, the model output "not sure"). Both the baseline max(logit) method and our uncertainty estimator select same number of confident images in the three subset: low, medium, high select 41k($\sim$ 82\%), 39k($\sim$ 79\%), 36k($\sim$ 73\%) ImageNet images respectively. 
% For our method, we find the 18\%, 21\%, 27\% least confident samples whose top-1 prediction has inconsistent inferred classes when applying $B=2, 4, 8$ different sets of $\mathcal{T}$, respectively.
% On the least confident subset that our method proposes to abstain, the accuracy is only 21.63\%, significantly lower than the overall average (See Table~\ref{table:zero-shot}). 
% (low=2 set, medium=4 set, and high=8 set) 
% to increase the confidence score threshold and more images are treated as "not sure". For max(logit) method, we set proper logit threshold to keep same number of confident samples as our method on each subset.


%      \# High confidence set  & 40776 & 39694 & 36505         & 40776 & 39694 & 36505\\
%      \% High confidence set  & 81.55\% & 79.39\% & 73.01\% &  81.55\% & 79.28\% &  73.10\% \\

% \todo{describe how you define low, medium, high confidence score.}
% Fig.~\ref{fig:select-pred-result} show that our confidence estimation method can help the model select another action, Not sure, when the model has low confidence for the decision. Here is the Accuracy vs Confidence table.




% \begin{minipage}{0.60\linewidth}
%     \centering
%     % \vspace{-30}
%     \includegraphics[width=2.8in]{fig/Fig-select-pred-result.pdf}
% \end{minipage}
% \begin{minipage}{0.39\linewidth}
%     % \vspace{-30}
%     \centering
%     \caption{Selective prediction results in Accuracy vs Confidence figure: our confidence estimation method can help the model select another action, Not sure, when the model has low confidence for the decision. }
% \label{fig:5}
% \end{minipage}

% \begin{figure}[t]
% \centering
% \includegraphics[width=0.5\textwidth]{fig/Fig-select-pred-result.pdf}
% \caption{ Selective prediction results in Accuracy vs Confidence figure: our uncertainty estimation method can help the model select another action, Not sure, when the model has low confidence for the decision. }
% \label{fig:select-pred-result}
% \end{figure}

\vspace{-3pt}
\subsection{Using hierarchy to help improve zero-shot accuracy on low confidence subset}
\vspace{-3pt}
Using top-down and bottom-up label augmentation significantly improves the accuracy on the low confident subset.
For the low confidence subset, we apply the top-down and bottom-up label augmentation method. 
Table~\ref{table:zero-shot} shows improvement of 16.97\% on the top-1 accuracy (from 21.58\% to 38.71\%) for the identified low confidence subset of samples, and overall 3.6\% on the top-1 accuracy (64.18\% to 67.78\%) for all samples in ImageNet.
We show similar improvement on the zero-shot accuracy for ImageNet shifted datasets. 
To investigate if our method works for other multi-modal models, we apply our method to the LiT \citep{zhai2022lit} model and observe that our method improves accuracy for LiT models as well. See appendix Fig.~\ref{fig:qualitative-result} for qualitative visualization. %In  LiT, the image encoder is pre-trained and ``locked'' and the text encoder is trained to align with the image encoder, so we believe that the LiT text encoder is more robust.       %Interestingly, we find the improvement on LiT is not as large as CLIP model, which may suggest that LiT model is more robust at prompt and image perturbations.  


% %%%%%%%%% 
% %%%%%%%%% table-1
% %%%%%%%%% 

% \begin{table*}[tp]
% %   \small
% %   \footnotesize
% % \scriptsize
% \centering
% % \vspace{-5pt}
% \caption{CLIP (ViT-B-16) and LiT (ViT-B-32) zero-shot Top-1 accuracy on various datasets (do not use prompts during decision)}
% %\rowcolors{2}{gray!25}{white}
% \begin{tabular}{c c |c c| c c}
%     \toprule
%  %   \rowcolor{LightCyan}
%      & & CLIP & (Ours) Hierarchy-CLIP & LiT & (Ours) Hierarchy-LiT\\
%     % iamgenet
%     \midrule
%      \multirow{2}{*}{ImageNet} & Low confidence subset  & 21.58\% & \bf{38.71\%}  & 31.18\% & \bf{37.25\%} \\ 
%      & Full dataset & 64.18\% & \bf{67.78\% } & 68.26\% & \bf{69.41\% }  \\ 
%  % \multirow{2}{*}{ImageNet} & Low confidence subset (9340) 

     
%      % iamgenet-v2
%     \midrule
%  %   \rowcolor{Gray}
%      \multirow{2}{*}{ImageNet-v2}& Low confidence subset  & 17.77\% & \bf{32.50\%} & 27.08\% & \bf{31.45\% }\\
%  %    \rowcolor{Gray}
%      & Full dataset  & 58.06\% & \bf{61.07\%} & 60.11\% & \bf{61.11\% } \\
    
%     % iamgenet-R
%     \midrule
%      \multirow{2}{*}{ImageNet-R} & Low confidence subset  & 16.79\% & \bf{27.91\% } & 21.82\% & \bf{22.93\% } \\
%      & Full dataset & 56.88\% & \bf{59.46\%} & 66.54\% & \bf{66.75\% }  \\
    
%     % iamgenet-Adversarial
%     \midrule
%  %  \rowcolor{Gray}
%      \multirow{2}{*}{ImageNet-Adversarial} & Low confidence subset  & 10.13\% & \bf{18.44\% } & 7.19\% & \bf{8.95\% }\\
%      & Full dataset & 26.12\% & \bf{29.23\% } & 13.93\% & \bf{14.56\%}  \\
     
%      % iamgenet-sketch
%     \midrule
% % \rowcolor{Gray}
%      \multirow{2}{*}{ImageNet-Sketch} & Low confidence subset & 13.74\% & \bf{23.18\% } & 21.51\% & \bf{24.42\%}\\
%      & Full dataset  & 44.71\% & \bf{47.28\% } & 52.47\% & \bf{53.17\% }  \\   
     
%      \bottomrule
% \end{tabular}
% \label{table:zero-shot}
% \end{table*}

%%%%%%%%% 
%%%%%%%%% table-1
%%%%%%%%% 


% We conduct experiment on two popular multi-modal model; CLIP and LiT.
% We conduct zero-shot classification (without any finetune) on the ImageNet dataset with CLIP (ViT-B-16) based models.  
% Similarly, we conduct same zero-shot classification (without any finetune) with LiT (ViT-B-32) based models. Table.~\ref{table:zero-shot} right two column shows the performance: we could find similar consistent improvement as CLIP model after using our method. 


%%%%%%%%% 
%%%%%%%%% table-2 after adding prompts
%%%%%%%%% 


\subsection{Ablation study}








\paragraph{Our hierarchy-based label augmentation is complimentary to prompt ensembling.}
Prompt ensembling requires a set of manually crafted prompt templates, and the zero-shot performance is sensitive to the set of prompts the model uses. 
Alternatively, our proposed method does not require a dedicated tuning of the prompt templates. We directly augment the class name with knowledge of the hierarchy. Our method is more straightforward and interpretable. 

To test if our hierarchy-based method is complimentary with prompt ensembling, after applying our top-down and bottom-up label augmentation, we additionally apply prompt ensembling. 
For the low confidence set, we first create a prompt template to transform the child and parent name pairs into a new class name $\tilde{c}$ in natural language: ``{\small\texttt{\{child\} which is a kind of \{parent\}}}''. Then we apply the 80 prompts designed by the CLIP paper \cite{radford2021learning} individually to the new class name $\tilde{c}$, and then ensemble them. 
For the high confidence set, since we do not modify the class name using hierarchy information, we only apply the prompt ensemble alone. 
The performance is shown in Table \ref{table:add_prompt}. We compare the zero-shot accuracy using the vanilla prompt ensemble method proposed in CLIP, and the zero-shot accuracy using our combined version of hierarchy-based class name augmentation and prompt ensembling. 
As shown in the table, using both hierarchy and prompt ensembling achieves better or on par accuracy with the prompt ensemble alone, suggesting that the two methods can be combined. 
Considering the prompt ensemble requires manually designed prompt templates and much greater inference time, our hierarchy-based class name augmentation is simple, efficient and effective. 




\paragraph{Effect of threshold of confidence score on zero-shot accuracy.}
In Table \ref{table:zero-shot} we use a binary criterion to determine the low confidence set. 
We can alternatively use the continuous confidence score by choosing a threshold based on the trade-off between precision and recall. 
Changing the threshold of the confidence score can lead to different numbers of samples in the low confidence set.
We study the effect of threshold on zero-shot accuracy. Table \ref{table:threshold} shows the overall accuracy with different thresholds. We find that the overall accuracy is relatively robust to the threshold selection, in the wide range from 0.47 to 0.70.



\begin{table}[tp]
%   \small
  \footnotesize
% \scriptsize
\centering
\vspace{-10pt}
\caption{Effect of threshold of confidence score on zero-shot accuracy. }
\scalebox{0.9}{%
%\rowcolors{2}{gray!25}{white}
\begin{tabular}{c c |c c}
    \toprule
 %   \rowcolor{LightCyan}
     Threshold & Low conf. set size & Acc of low conf. set & Acc of full set \\
    % iamgenet
    \midrule
     0.47 & 10000  & 19.40\% & 68.72\%  \\ 
     0.52 & 11000 & 20.82\% & 68.78\%   \\
     0.57 & 12000  & 22.06\% & 68.82\%  \\ 
     0.62 & 13000 &  23.58\% &    68.85\%  \\ 
     0.66 & 14000 &  25.01\% &    \bf{68.88}\%  \\ 
     0.70 & 15000 &  26.51\% &    68.86\%  \\ 
    
     \bottomrule
\end{tabular}
}
\label{table:threshold}
\vspace{-8pt}
\end{table}


\paragraph{Effect of WordNet sparsity on zero-shot accuracy}
We evaluate the effect of the degree of sparsity of WordNet on the downstream zero-shot accuracy. 
%We fix the size of the selected Low confident set as 10000 images.
The results we show in the previous sections are based on the sparsified WordNet which only keeps 40\% of nodes with high word frequency. 
Here we study the effect of this threshold on the downstream zero-shot accuracy. 
Table~\ref{table:threshold-wordnet} shows the overall accuracy with different thresholds for WordNet sparsity. 


\begin{table}[tp]
%   \small
  \footnotesize
% \scriptsize
\centering
% \vspace{-5pt}
\caption{Effect of WordNet sparsity on zero-shot accuracy}
\scalebox{0.9}{%
%\rowcolors{2}{gray!25}{white}
\begin{tabular}{c c c}
    \toprule
 %   \rowcolor{LightCyan}
     \% of remaining words & acc overall\\
    % iamgenet
    \midrule
    100\%  &  68.52\%  \\ 
     40\%   &  68.52\%  \\ 
     30\%  &  \bf{68.72}\%   \\
     20\%   &  \bf{68.72}\%  \\ 
     10\%   &  \bf{68.72}\%  \\
     \bottomrule
\end{tabular}
}
\label{table:threshold-wordnet}
\vspace{-12pt}
\end{table}



% \paragraph{Influence of sample of prompts consistency}


\section{Conclusion}
% \todo{need modify}
Multi-modal models' generalization and robustness is critical for deployment. %Currently the multi-modal’s zero-shot accuracy is still much lower than the production standard. 
Motivated by the big gap between top-1 and top-5 accuracy in ImageNet zero-shot classification, we investigated the failure modes and found that the model's prediction is very sensitive to text prompts. 
We describe a simple but efficient zero-shot post-hoc method to identify a subset of samples that are most likely to be predicted wrongly a measure of self-consistency.
For those in the low confidence subset, we use the WordNet hierarchy to augment class labels to enhance the robustness, resulting in up to 17.13\% accuracy improvement.  
We show our method provides consistent improvement over other distribution shifted datasets, and is generalizable to other image-text models.
% but may also their robustness, generalization, and calibration, which can lead to more reliable and trustworthy decisions. 
% Overall, our proposed method shows significant improvement on accuracy and generalization for zero-shot inference. 
% Our framework is hyperparameter-free, training-free, post-processing method that can be easily extended to other multi-modal architectures.






% %%%%%%%%% 
% %%%%%%%%% table-2 after adding prompts
% %%%%%%%%% 

% \begin{table*}[tp]
% %   \small
% %   \footnotesize
% % \scriptsize
% \centering
% % \vspace{-5pt}
% \caption{CLIP (ViT-B-16) and LiT (ViT-B-32) zero-shot Top-1 accuracy on various datasets ((use prompts during decision))}
% %\rowcolors{2}{gray!25}{white}
% \begin{tabular}{c c |c c| c c}
%     \toprule
%  %   \rowcolor{LightCyan}
%      & & CLIP & (Ours) Hierarchy-CLIP & LiT & (Ours) Hierarchy-LiT\\
%     % iamgenet
%     \midrule
%      \multirow{2}{*}{ImageNet} & Low confidence subset  & 24.41\% & \bf{41.22\%}  & \% & \bf{\%} \\ 
%      & Full dataset & 68.48\% & \bf{68.90\% } & \% & \bf{\% }  \\ 
%  % \multirow{2}{*}{ImageNet} & Low confidence subset (9340) 

     
%      % iamgenet-v2
%     \midrule
%  %   \rowcolor{Gray}
%      \multirow{2}{*}{ImageNet-v2}& Low confidence subset  &  \% & \bf{ \%} &  \% & \bf{ \% }\\
%  %    \rowcolor{Gray}
%      & Full dataset  &  62.02\% & \bf{ 62.05\%} &  \% & \bf{\% } \\
    
%     % iamgenet-R
%     \midrule
%      \multirow{2}{*}{ImageNet-R} & Low confidence subset  &  \% & \bf{ \% } &  \% & \bf{ \% } \\
%      & Full dataset &  60.21\% & \bf{ 60.57\%} &  \% & \bf{ \% }  \\
    
%     % iamgenet-Adversarial
%     \midrule
%  %  \rowcolor{Gray}
%      \multirow{2}{*}{ImageNet-Adversarial} & Low confidence subset  &  \% & \bf{ \% } &  \% & \bf{ \% }\\
%      & Full dataset &  30.59\% & \bf{ 31.15\% } &  \% & \bf{ \%}  \\
     
%      % iamgenet-sketch
%     \midrule
% % \rowcolor{Gray}
%      \multirow{2}{*}{ImageNet-Sketch} & Low confidence subset &  \% & \bf{ \% } &  \% & \bf{ \%}\\
%      & Full dataset  &  48.52\% & \bf{ \% } &  \% & \bf{ \% }  \\   
     
%      \bottomrule
% \end{tabular}
% \label{table:zero-shot}
% % \vspace{-12pt}
% \end{table*}








% \vspace{-0.5em}
% \section{Related work}
% % \vspace{-0.5em}
% % \paragraph{Prompt engineering and learning}
% % Our re-ranking method essentially leverages the rich label hierarchy to craft the prompts, therefore is related to prompt engineering.
% %
% Prompt engineering and learning has attracted much attention in vision and learning since the introduction of image-text models \citep{radford2021learning, jia2021scaling, zhai2022lit}. 
% %
% The image-text models align images and their text descriptions into a common space, which facilitates the model to generalize to unseen categories in the inference time. 
% %
% However, it has been observed that the downstream image classification accuracy highly depends on the input prompts. 
% %
% This motivates researchers to either fine-tune or auto-learn prompts when adapting multi-modal models to downstream vision tasks.

% \citet{zhou2022learning, zhou2022conditional} propose CoOp and CoCoOp to automatically learn the prompt word embeddings in the few-shot settings, and show significant improvements over the vanilla zero-shot image classification based-on prompting. 
% %
% %MH: learning? or supervised?
% These are learning based approaches, requiring label supervised data from downstream tasks, while our proposed method is zero-shot and post-hoc without using any supervised data. 
% %
% % In contrast, \citet{radford2021learning} suggest different approaches for prompt engineering.
% % %
% % %MH: I do not understand this sentence 
% % For generic object and scenes, using template ``a photo of \{class\}''; for fine-grained categorization, type related context is added, e.g., ``a type of food'' for Food101. All the suggested crafting only changes the context, but fix the ``class'' in the template. Our method is different from them in that we fix the context, but only adapt the ``class''.
% In concurrent work, \citet{shu2022test} propose to learn the prompt embedding in an unsupervised manner by minimizing the entropy of the averaged prediction probability distribution, where each prediction is based on a random augmentation applied to the input image.
% Our work is different from \citep{shu2022test} in the sense that we do not learn an input-dependent prompt embedding. Instead we only selectively modify the prompts using knowledge hierarchy for images that have unreliable predictions, and our modified new prompt is natural language not numerical values. 


%%%%%%%%% 
%%%%%%%%% 
%%%%%%%%%  CLIP model
%%%%%%%%% 
%%%%%%%%% 
% \subsubsection{CLIP model}
% \noindent{\bf CLIP model} We conduct zero-shot classification (without any finetune) on the ImageNet dataset with CLIP based models. Here are the performance.
% \todo{specify architecture which CLIP model}

% \noindent{\bf LiT model} 
% We conduct zero-shot classification (without any finetune) on the ImageNet dataset with LiT based models. Here are the performance. \todo{specify which LiT model you used}





% \begin{table}[tp]
%   \small
% %   \footnotesize
% % \scriptsize
% \centering
% % \vspace{-5pt}
% \caption{LiT zero-shot Top-1 accuracy on different datasets}
% \begin{tabular}{c c |c c}
%     \toprule
%      & & CLIP zero-shot & (Ours) Hierarchy-CLIP zero-shot\\
%     % iamgenet
%     \midrule
%     \multirow{2}{*}{ImageNet} & Low confidence subset (9340) & 31.18\% & \bf{37.25\% ( +6.1\%)} \\
%      & Full dataset (50000) & 68.26\% & \bf{69.41\% ( +1.15\%)}  \\
 
%      % iamgenet-v2
%     \midrule
%      \multirow{2}{*}{ImageNet-v2} & Low confidence subset (2286) & 27.08\% & \bf{31.45\% (+4.37\%)} \\
%      & Full dataset (10000) & 60.11\% & \bf{61.11\% (+1.00\%)}  \\
    
%     % iamgenet-R
%     \midrule
%      \multirow{2}{*}{ImageNet-R} & Low confidence subset (5656) & 21.82\% & \bf{22.93\% (+1.11\%)} \\
%      & Full dataset (30000) & 66.54\% & \bf{66.75\% (+0.21\%)}  \\
    
%     % iamgenet-Adversarial
%     \midrule
%      \multirow{2}{*}{ImageNet-Adversarial} & Low confidence subset (2671) & 7.19\% & \bf{8.95\% (+1.76\%)} \\
%      & Full dataset (7500) & 13.93\% & \bf{14.56\% (+0.63\%)}  \\
     
%      % iamgenet-sketch
%     \midrule
%      \multirow{2}{*}{ImageNet-Sketch} & Low confidence subset (12248) & 21.51\% & \bf{24.42\% (+2.91\%)} \\
%      & Full dataset (50889) & 52.47\% & \bf{53.17\% (+0.7\%)}  \\  
     
%      \bottomrule
% \end{tabular}
% \label{table:skill}
% % \vspace{-12pt}
% \end{table}


% \begin{table}[tp]
%   \small
% %   \footnotesize
% % \scriptsize
% \centering
% % \vspace{-5pt}
% \caption{CLIP (ViT-B-16) zero-shot Top-1 accuracy on various datasets}
% %\rowcolors{2}{gray!25}{white}
% \begin{tabular}{c c |c c}
%     \toprule
%  %   \rowcolor{LightCyan}
%      & & CLIP zero-shot & (Ours) Hierarchy-CLIP zero-shot\\
%     % iamgenet
%     \midrule
%      \multirow{2}{*}{ImageNet} & Low confidence subset (10327) & 21.58\% & \bf{38.71\% (+17.13\%)} \\
%      & Full dataset (50000) & 64.18\% & \bf{67.78\% (+3.60\%)}  \\
 
%      % iamgenet-v2
%     \midrule
%  %   \rowcolor{Gray}
%      \multirow{2}{*}{ImageNet-v2}& Low confidence subset (2043) & 17.77\% & \bf{32.50\% (+14.73\%)} \\
%  %    \rowcolor{Gray}
%      & Full dataset (10000) & 58.06\% & \bf{61.07\% (+3.01\%)}  \\
    
%     % iamgenet-R
%     \midrule
%      \multirow{2}{*}{ImageNet-R} & Low confidence subset (6969) & 16.79\% & \bf{27.91\% (+11.12\%)} \\
%      & Full dataset (30000) & 56.88\% & \bf{59.46\% (+2.58\%)}  \\
    
%     % iamgenet-Adversarial
%     \midrule
%  %  \rowcolor{Gray}
%      \multirow{2}{*}{ImageNet-Adversarial} & Low confidence subset (2803) & 10.13\% & \bf{18.44\% (+8.31\%)} \\
%      & Full dataset (7500) & 26.12\% & \bf{29.23\% (+3.11\%)}  \\
     
%      % iamgenet-sketch
%     \midrule
% % \rowcolor{Gray}
%      \multirow{2}{*}{ImageNet-Sketch} & Low confidence subset (13875) & 13.74\% & \bf{23.18\% (+9.44\%)} \\
%      & Full dataset (50889) & 44.71\% & \bf{47.28\% (+2.57\%)}  \\   
     
%      \bottomrule
% \end{tabular}
% \label{table:skill}
% % \vspace{-12pt}
% \end{table}


% %%%%%%%%% 
% %%%%%%%%% table-1
% %%%%%%%%% 

% \begin{table}[tp]
% %   \small
% %   \footnotesize
% % \scriptsize
% \centering
% % \vspace{-5pt}
% \caption{Hierarchy-CLIP Top-1 accuracy on ImageNet}
% \begin{tabular}{c |c c}
%     \toprule
%     ImageNet & CLIP Top-1 zero-shot acc & (Ours) Hierarchy-CLIP Top-1 zero-shot acc\\
%     \midrule
%      Low confidence subset (10327) & 21.58\% & \bf{38.71\% (17.13\% improvement)} \\
%      Full dataset (50k) & 64.18\% & \bf{67.78\% (3.60\% improvement)}  \\
%      \bottomrule
% \end{tabular}
% \label{table:skill}
% % \vspace{-12pt}
% \end{table}


% %%%%%%%%% 
% %%%%%%%%% table-2
% %%%%%%%%% 

% \begin{table}[tp]
% %   \small
% %   \footnotesize
% % \scriptsize
% \centering
% % \vspace{-5pt}
% \caption{Hierarchy-CLIP Top-1 accuracy on ImageNet-v2}
% \begin{tabular}{c |c c}
%     \toprule
%     ImageNet-v2 & CLIP Top-1 zero-shot acc & (Ours) Hierarchy-CLIP Top-1 zero-shot acc\\
%     \midrule
%      Low confidence subset (2043) & 17.77\% & \bf{32.50\% (14.73\% improvement)} \\
%      Full dataset (10k) & 58.06\% & \bf{61.07\% (3.01\% improvement)}  \\
%      \bottomrule
% \end{tabular}
% \label{table:skill}
% % \vspace{-12pt}
% \end{table}

% %%%%%%%%% 
% %%%%%%%%% table-3
% %%%%%%%%% 

% \begin{table}[tp]
% %   \small
% %   \footnotesize
% % \scriptsize
% \centering
% % \vspace{-5pt}
% \caption{Hierarchy-CLIP Top-1 accuracy on ImageNet-R}
% \begin{tabular}{c |c c}
%     \toprule
%     ImageNet-R & CLIP Top-1 zero-shot acc & (Ours) Hierarchy-CLIP Top-1 zero-shot acc\\
%     \midrule
%      Low confidence subset (6969) & 16.79\% & \bf{27.91\% (11.12\% improvement)} \\
%      Full dataset (30k) & 56.88\% & \bf{59.46\% (2.58\% improvement)}  \\
%      \bottomrule
% \end{tabular}
% \label{table:skill}
% % \vspace{-12pt}
% \end{table}


% %%%%%%%%% 
% %%%%%%%%% table-4
% %%%%%%%%% 

% \begin{table}[tp]
% %   \small
% %   \footnotesize
% % \scriptsize
% \centering
% % \vspace{-5pt}
% \caption{Hierarchy-CLIP Top-1 accuracy on ImageNet-Adversarial}
% \begin{tabular}{c |c c}
%     \toprule
%     ImageNet-Adversarial & CLIP Top-1 zero-shot acc & (Ours) Hierarchy-CLIP Top-1 zero-shot acc\\
%     \midrule
%      Low confidence subset (2803) & 10.13\% & \bf{18.44\% (8.31\% improvement)} \\
%      Full dataset (7500) & 26.12\% & \bf{29.23\% (3.11\% improvement)}  \\
%      \bottomrule
% \end{tabular}
% \label{table:skill}
% % \vspace{-12pt}
% \end{table}

% %%%%%%%%% 
% %%%%%%%%% table-5
% %%%%%%%%% 

% \begin{table}[tp]
% %   \small
% %   \footnotesize
% % \scriptsize
% \centering
% % \vspace{-5pt}
% \caption{Hierarchy-CLIP Top-1 accuracy on ImageNet-Sketch}
% \begin{tabular}{c |c c}
%     \toprule
%     ImageNet-Sketch & CLIP Top-1 zero-shot acc & (Ours) Hierarchy-CLIP Top-1 zero-shot acc\\
%     \midrule
%      Low confidence subset (13875) & 13.74\% & \bf{23.18\% (9.44\% improvement)} \\
%      Full dataset (50889) & 44.71\% & \bf{47.28\% (2.57\% improvement)}  \\
%      \bottomrule
% \end{tabular}
% \label{table:skill}
% % \vspace{-12pt}
% \end{table}

% %%%%%%%%% 
% %%%%%%%%% table-6
% %%%%%%%%% 

% \begin{table}[tp]
% %   \small
% %   \footnotesize
% % \scriptsize
% \centering
% % \vspace{-5pt}
% \caption{Hierarchy-CLIP Top-1 accuracy on ObjectNet}
% \begin{tabular}{c |c c}
%     \toprule
%     ObjectNet & CLIP Top-1 zero-shot acc & (Ours) Hierarchy-CLIP Top-1 zero-shot acc\\
%     \midrule
%      Low confidence subset & 0\% & \bf{0\% ($\sim$ 0\% improvement)} \\
%      Full dataset & 0\% & \bf{0\% ($\sim$ 0\% improvement)}  \\
%      \bottomrule
% \end{tabular}
% \label{table:skill}
% % \vspace{-12pt}
% \end{table}




%%%%%%%%% 
%%%%%%%%% 
%%%%%%%%%  LiT model
%%%%%%%%% 
%%%%%%%%% 

% \subsubsection{LiT model}


%%%%%%%%% 
%%%%%%%%% table-1
%%%%%%%%% 

% \begin{table}[tp]
%   \small
% %   \footnotesize
% % \scriptsize
% \centering
% % \vspace{-5pt}
% \caption{LiT zero-shot Top-1 accuracy on different datasets}
% \begin{tabular}{c c |c c}
%     \toprule
%      & & CLIP zero-shot & (Ours) Hierarchy-CLIP zero-shot\\
%     % iamgenet
%     \midrule
%     \multirow{2}{*}{ImageNet} & Low confidence subset (9340) & 31.18\% & \bf{37.25\% ( +6.1\%)} \\
%      & Full dataset (50000) & 68.26\% & \bf{69.41\% ( +1.15\%)}  \\
 
%      % iamgenet-v2
%     \midrule
%      \multirow{2}{*}{ImageNet-v2} & Low confidence subset (2286) & 27.08\% & \bf{31.45\% (+4.37\%)} \\
%      & Full dataset (10000) & 60.11\% & \bf{61.11\% (+1.00\%)}  \\
    
%     % iamgenet-R
%     \midrule
%      \multirow{2}{*}{ImageNet-v2} & Low confidence subset (5656) & 21.82\% & \bf{22.93\% (+1.11\%)} \\
%      & Full dataset (30000) & 66.54\% & \bf{66.75\% (+0.21\%)}  \\
    
%     % iamgenet-Adversarial
%     \midrule
%      \multirow{2}{*}{ImageNet-Adversarial} & Low confidence subset (2671) & 7.19\% & \bf{8.95\% (+1.76\%)} \\
%      & Full dataset (7500) & 13.93\% & \bf{14.56\% (+0.63\%)}  \\
     
%      % iamgenet-sketch
%     \midrule
%      \multirow{2}{*}{ImageNet-Sketch} & Low confidence subset (12248) & 21.51\% & \bf{24.42\% (+2.91\%)} \\
%      & Full dataset (50889) & 52.47\% & \bf{53.17\% (+0.7\%)}  \\  
     
%      \bottomrule
% \end{tabular}
% \label{table:skill}
% % \vspace{-12pt}
% \end{table}




% %%%%%%%%% 
% %%%%%%%%% table-1
% %%%%%%%%% 

% \begin{table}[tp]
% %   \small
% %   \footnotesize
% % \scriptsize
% \centering
% % \vspace{-5pt}
% \caption{Hierarchy-LiT Top-1 accuracy on ImageNet}
% \begin{tabular}{c |c c}
%     \toprule
%     ImageNet & LiT Top-1 zero-shot acc & (Ours) Hierarchy-LiT Top-1 zero-shot acc\\
%     \midrule
%      Low confidence subset (9340) & 31.18\% & \bf{37.25\% ( 6.1\% improvement)} \\
%      Full dataset (50000) & 68.26\% & \bf{69.41\% ( 1.15\% improvement)}  \\
%      \bottomrule
% \end{tabular}
% \label{table:skill}
% % \vspace{-12pt}
% \end{table}


% %%%%%%%%% 
% %%%%%%%%% table-2
% %%%%%%%%% 

% \begin{table}[tp]
% %   \small
% %   \footnotesize
% % \scriptsize
% \centering
% % \vspace{-5pt}
% \caption{Hierarchy-LiT Top-1 accuracy on ImageNet-v2}
% \begin{tabular}{c |c c}
%     \toprule
%     ImageNet-v2 & LiT Top-1 zero-shot acc & (Ours) Hierarchy-LiT Top-1 zero-shot acc\\
%     \midrule
%      Low confidence subset (2286) & 27.08\% & \bf{31.45\% (4.37\% improvement)} \\
%      Full dataset (10000) & 60.11\% & \bf{61.11\% (1.00\% improvement)}  \\
%      \bottomrule
% \end{tabular}
% \label{table:skill}
% % \vspace{-12pt}
% \end{table}

% %%%%%%%%% 
% %%%%%%%%% table-3
% %%%%%%%%% 

% \begin{table}
% %   \small
% %   \footnotesize
% % \scriptsize
% \centering
% % \vspace{-5pt}
% \caption{Hierarchy-LiT Top-1 accuracy on ImageNet-R}
% \begin{tabular}{c |c c}
%     \toprule
%     ImageNet-R & LiT Top-1 zero-shot acc & (Ours) Hierarchy-LiT Top-1 zero-shot acc\\
%     \midrule
%      Low confidence subset (5656) & 21.82\% & \bf{22.93\% (1.11\% improvement)} \\
%      Full dataset (30000) & 66.54\% & \bf{66.75\% (0.21\% improvement)}  \\
%      \bottomrule
% \end{tabular}
% \label{table:skill}
% % \vspace{-12pt}
% \end{table}

% %%%%%%%%% 
% %%%%%%%%% table-4
% %%%%%%%%% 

% \begin{table}
% %   \small
% %   \footnotesize
% % \scriptsize
% \centering
% % \vspace{-5pt}
% \caption{Hierarchy-LiT Top-1 accuracy on ImageNet-Adversarial}
% \begin{tabular}{c |c c}
%     \toprule
%     ImageNet-Adversarial & LiT Top-1 zero-shot acc & (Ours) Hierarchy-LiT Top-1 zero-shot acc\\
%     \midrule
%      Low confidence subset (2671) & 7.19\% & \bf{8.95\% (1.76\% improvement)} \\
%      Full dataset (7500) & 13.93\% & \bf{14.56\% (0.63\% improvement)}  \\
%      \bottomrule
% \end{tabular}
% \label{table:skill}
% % \vspace{-12pt}
% \end{table}

% %%%%%%%% 
% %%%%%%%% table-5
% %%%%%%%% 

% \begin{table}
% %   \small
% %   \footnotesize
% % \scriptsize
% \centering
% % \vspace{-5pt}
% \caption{Hierarchy-LiT Top-1 accuracy on ImageNet-Sketch}
% \begin{tabular}{c |c c}
%     \toprule
%     ImageNet-Sketch & LiT Top-1 zero-shot acc & (Ours) Hierarchy-LiT Top-1 zero-shot acc\\
%     \midrule
%      Low confidence subset (12248) & 21.51\% & \bf{24.42\% (2.91\% improvement)} \\
%      Full dataset (50889) & 52.47\% & \bf{53.17\% (0.7\% improvement)}  \\
%      \bottomrule
% \end{tabular}
% \label{table:skill}
% % \vspace{-12pt}
% \end{table}







% %%%%%%%% 
% %%%%%%%% table-select-pred-result
% %%%%%%%% 

% \begin{table}
% %   \small
% %   \footnotesize
% \scriptsize
% \centering
% % \vspace{-5pt}
% \caption{Hierarchy-CLIP Top-1 Accuracy vs Confidence on ImageNet \todo{convert to a line plot}}
% \begin{tabular}{c |c c c | c c c}
%     \toprule
%   & \multicolumn{3}{c}{Our uncertainty estimator } & \multicolumn{3}{c}{Max(logit) }\\
%     Confidence score $\tau$ & low & medium & high &  low & medium & high\\
%     \midrule
%      \# High confidence set  & 40776 & 39694 & 36505         & 40776 & 39694 & 36505\\
%      \% High confidence set  & 81.55\% & 79.39\% & 73.01\% &  81.55\% & 79.28\% &  73.10\% \\
%      Top-1 accuracy on samples with confidence score  $>\tau$ & \textbf{74.15\%} & \textbf{75.23\%} & \textbf{78.33\%} & 68.95\% & 69.38\% & 70.73\%\\
%     %  Top-1 accuracy on samples with confidence score  $<\tau$ & \textbf{20.09\%} & \textbf{21.63\%} & \textbf{25.91\%}  & 43.21\% & 44.21\% & 46.46\%\\
%      \bottomrule
% \end{tabular}
% \label{table:select}
% % \vspace{-12pt}
% \end{table}


% %%%%%%%% 
% %%%%%%%% table-5
% %%%%%%%% 

% \begin{table}
% %   \small
% %   \footnotesize
% \scriptsize
% \centering
% % \vspace{-5pt}
% \caption{Hierarchy-CLIP Top-1 Accuracy vs Confidence on ImageNet \todo{convert to a line plot}}
% \begin{tabular}{c |c c c | c c c}
%     \toprule
%   & \multicolumn{3}{c}{Our uncertainty estimator } & \multicolumn{3}{c}{Max(logit) }\\
%     Confidence score $\tau$ & low & medium & high &  low & medium & high\\
%     \midrule
%      \# High confidence set  & 40776 & 39694 & 36505   & 40687 & 39638 & 36552\\
%      \% High confidence set  & 81.55\% & 79.39\% & 73.01\% &  81.37\% & 79.28\% &  73.10\% \\
%      Top-1 accuracy on samples with confidence score  $>\tau$ & \textbf{74.15\%} & \textbf{75.23\%} & \textbf{78.33\%} & 68.98\% & 69.40\% & 70.70\%\\
%     %  Top-1 accuracy on samples with confidence score  $<\tau$ & \textbf{20.09\%} & \textbf{21.63\%} & \textbf{25.91\%}  & 43.21\% & 44.21\% & 46.46\%\\
%      \bottomrule
% \end{tabular}
% \label{table:select}
% % \vspace{-12pt}
% \end{table}

% %%%%%%%% 
% %%%%%%%% table-5
% %%%%%%%% 

% \begin{table}
%   \small
% %   \footnotesize
% % \scriptsize
% \centering
% % \vspace{-5pt}
% \caption{Hierarchy-CLIP Top-1 Accuracy vs Confidence on ImageNet}
% \begin{tabular}{c |c c c c}
%     \toprule
%     Confidence score $\tau$ & low & medium & high & \\
%     \midrule
%      \# High confidence set  & 40776 & 39694 & 36505 \\
%      \% High confidence set  & 81.55\% & 79.39\% & 73.01\% \\
%      Top-1 accuracy on samples with confidence score  $>\tau$ & 74.15\% & 75.23\% & 78.33\%\\
%      Top-1 accuracy on samples with confidence score  $<\tau$ & 20.09\% & 21.63\% & 25.91\%\\
%      \bottomrule
% \end{tabular}
% \label{table:select}
% % \vspace{-12pt}
% \end{table}


% %%%%%%%% 
% %%%%%%%% table-5
% %%%%%%%% 

% \begin{table}
%   \small
% %   \footnotesize
% % \scriptsize
% \centering
% % \vspace{-5pt}
% \caption{CLIP Top-1 Accuracy vs Confidence on ImageNet, we use different threshold $\tau$ to select samples that Max(logic) $ > \tau$}
% \begin{tabular}{c |c c c c}
%     \toprule
%     Confidence score $\tau$ & low & medium & high & \\
%     \midrule
%      \# High confidence set  & 40687 & 39638 & 36552  \\
%      \% High confidence set  &  81.37\% & 79.28\% &  73.10\% \\
%      Top-1 accuracy on samples with confidence score  $>\tau$ & 68.98\% & 69.40\% & 70.70\%\\
%      Top-1 accuracy on samples with confidence score  $<\tau$ & 43.21\% & 44.21\% & 46.46\%\\
%      \bottomrule
% \end{tabular}
% \label{table:select}
% % \vspace{-12pt}
% \end{table}

%%%%%%%%% 
%%%%%%%%% 
%%%%%%%%%  Ablation study
%%%%%%%%% 
%%%%%%%%% 

% \subsection{Ablation study}


% \subsubsection{Influence of number of children used in bottom-up hierarchy}


% \subsubsection{Influence of Lowest common ancestor or common ancestor used in top-up hierarchy}


% \subsubsection{Different method to sparse wordNet}

% \section{Conclusion}

% Multi-modal’s generalization and robustness is critical for deployment of the model to products. %Currently the multi-modal’s zero-shot accuracy is still much lower than the production standard. 
% Motivated by the big gap between top-1 accuracy and top-5 accuracy in zero-shot ImageNet inference, we investigated the failure modes and found that the model's prediction is very sensitive to text prompts. 
% Thus we develop a simple but efficient zero-shot post-hoc method to identify images where top prediction is unstable w.r.t. prompts. 
% For those unstable predictions, we make use of WordNet hierarchy to augment class labels to enhance the robustness, and that leads to up to 17.13\% improvement on accuracy.  
% We show our method make consistent improvement on other ImageNet shifted datasets and other model architectures.
% % but may also their robustness, generalization, and calibration, which can lead to more reliable and trustworthy decisions. 
% Overall, our proposed method shows significant improvement on accuracy and generalization for zero-shot inference. 
% Our framework is hyperparameter-free, training-free, post-processing method that can be easily extended to other multi-modal architectures. 




